MB-RACS: Measurement-Bounds-based Rate-Adaptive Image Compressed Sensing Network

Conventional compressed sensing (CS) algorithms typically apply a uniform sampling rate to different image blocks. A more strategic approach could be to allocate the number of measurements adaptively, based on each image block's complexity. In this paper, we propose a Measurement-Bounds-based Rate-Adaptive Image Compressed Sensing Network (MB-RACS) framework, which aims to adaptively determine the sampling rate for each image block in accordance with traditional measurement bounds theory. Moreover, since in real-world scenarios statistical information about the original image cannot be directly obtained, we suggest a multi-stage rate-adaptive sampling strategy. This strategy sequentially adjusts the sampling ratio allocation based on the information gathered from previous samplings. We formulate the multi-stage rate-adaptive sampling as a convex optimization problem and address it using a combination of Newton's method and binary search techniques. Additionally, we enhance our decoding process by incorporating skip connections between successive iterations to facilitate a richer transmission of feature information across iterations. Our experiments demonstrate that the proposed MB-RACS method surpasses current leading methods, with experimental evidence also underscoring the effectiveness of each module within our proposed framework.

==> Section/abstract_old.tex <==
\begin{abstract}
    In the field of image Compressed Sensing, recent studies have shown that neural networks can effectively assign different measurement numbers to image blocks, outperforming uniform allocation. Nonetheless, selecting measurement numbers is a high-dimensional discrete optimization problem. Neural network learning transforms this problem into a continuous optimization problem, but this approach only approximates the local optimal solution through gradient descent. In this paper, we propose the Measurement-Bounds-based Adaptive Compressed Sensing Network (MB-ACSNet), which determines measurement numbers based on measurement bounds derived from traditional Compressed Sensing. This method correlates sparsity to the number of measurements via mathematical proofs, providing a statistical solution that is more robust and generalizable compared to data-driven methods. For practical applications where the original image's sparsity information is unavailable, we implemented a two-stage approach and employed a network to predict the measurement bounds. Additionally, we devised a light-weight decoding network to accelerate the decoding process. Experimental results demonstrate that MB-ACSNet achieves better performance than existing deep learning-based image CS methods while maintaining a fast decoding speed.
\end{abstract}


==> Section/experiments_and_results_section/draft.tex <==
\iffalse
\paragraph{Experimental Results of Multi-Stage Rate-Adaptive Sampling}

We compare the multi-stage rate-adaptive sampling methods of MB-RAICS and CASNet. CASNet includes a two-stage rate-adpative sampling strategy. In the first sampling stage, it performs uniform sampling, and then, based on the information from the first stage, infers the saliency map and deploys the second stage's rate-adaptive sampling. Tab. \ref{tab:multi-stage-sampling-based comparison with CASNet on seven datasets} presents the PSNR and SSIM results of both methods across seven datasets at seven different sampling rates. In the case where the number of sampling stages is 2, MB-RAICS$_\text{i;2}$ outperforms CASNet$_\text{i;2}$ in PSNR/SSIM metrics by an average of 0.90dB/0.0141. In addition, increasing the number of sampling stages can boost performance; however, there's a diminishing return on this enhancement. For instance, MB-RAICS$_\text{i;5}$, having 5 sampling stages, outperforms the 2-stage version by an average of 0.29dB/0.0022 in PSNR/SSIM metrics. Yet, transitioning from MB-RAICS$_\text{i;5}$ to MB-RAICS$_\text{i;8}$ yields only an incremental average benefit of 0.05dB/0.0004. The performance improvement plateaus at 8 stages, as moving from 8 to 10 stages sees only a slight rise of 0.01dB/0.0002 in these metrics.
\fi

==> Section/experiments_and_results_section/experiments_and_results_drafts.tex <==
\begin{table*}
\centering
\caption{PSNR and SSIM comparisons for MB-RAICS and 8 baselines across Set11, CBSD68, Set5, Set14, BSDS100, Urban100, and Kodak24 datasets at sampling rates of 0.01, 0.04, 0.1, 0.25, 0.3, 0.4, and 0.5.}
\label{tab:comparison with state-of-the-arts methods}
\begin{tabular}{c c c c c c c c c c c c c c c c}
\toprule
\multirow{2}{*}[-1em]{Dataset} & \multirow{2}{*}[-1em]{Method} & \multicolumn{14}{c}{Sampling Ratio} \\ \cmidrule(lr){3-16} 
& & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.04} & \multicolumn{2}{c}{0.1} & \multicolumn{2}{c}{0.25} & \multicolumn{2}{c}{0.3} & \multicolumn{2}{c}{0.4} & \multicolumn{2}{c}{0.5} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16} & & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
\midrule
\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{Set11} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule

\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{CBSD68} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule

 \specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{Set5} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule

  \specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{Set5} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule

  \specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{Set5} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule

  \specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{Set5} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule

  \specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[-2em]{Set5} & CSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & ISTA-Net$^+$ & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & SCSNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & OPINE-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & AMP-Net & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & COAST & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & TransCS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & CASNet & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \cmidrule(l){2-16}
 & MB-RAICS & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\ \midrule
 \end{tabular}
\end{table*}

==> Section/experiments_and_results_section/experiments_and_results_old.tex <==
\section{Experiments and Results}\label{sec:experiment_and_result}

\subsection{Experimental Setup}
\label{sec:4:experimental setup}

\subsubsection{Datasets}
\label{sec:4:experimental setup:datasets}
Our training set aligns with \cite{8765626}. On 400 images from the training and test datasets of the BSDS500 database \cite{5557884}, we applied 8 data augmentation techniques. These images were then cropped into 96 × 96 sub-images, yielding a training set of 89,600 sub-images. Moreover, we conducted test experiments on seven datasets: Set11 \cite{Kulkarni_2016_CVPR}, CBSD68 \cite{937655}, Set5 \cite{bevilacqua2012low}, Set14 \cite{zeyde2012single}, BSDS100 \cite{937655}, Urban100 \cite{huang2015single}, and Kodak24 \cite{franzen1999kodak}. These datasets are commonly used as test sets in image compressive sensing and other image processing fields, containing images that range in number from a few to 100.

\input{Section/experiments_and_results_section/figures/single-stage_figure_different_methods_visual_results_sampling_rate_0.1}
\input{Section/experiments_and_results_section/figures/single-stage_figure_different_methods_visual_results_sampling_rate_0.01}

\subsubsection{Evaluation Metrics}
\label{sec:4:experimental setup:metrics}
We utilize two primary metrics to assess image quality and signal distortion in our experiments. Specifically, the peak signal-to-noise ratio (PSNR) provides a standard measure of reconstruction fidelity, while the multi-scale structural similarity (MS-SSIM) \cite{wang2003multiscale} offers insights into perceived image quality across different scales.

\subsubsection{Baselines}
\label{sec:4:experimental setup:baselines}

We compare the MB-RAICS with 8 baselines: CSNet \cite{8765626}, ISTA-Net$^+$ \cite{Zhang_2018_CVPR}, SCSNet \cite{Shi_2019_CVPR}, OPINE-Net \cite{9019857}, AMP-Net \cite{9298950}, COAST \cite{9467810}, TransCS \cite{9934025}, and CASNet \cite{9854112}. 
CSNet is a purely network-based method. ISTA-Net$^+$, OPINE-Net, AMP-Net, and TransCS are deep-unfolding-based methods. SCSNet achieves a scalable sampling rate through a scalable convolutional neural network. COAST allows sampling to generalize to any measurement matrix. CASNet designs a rate-adaptive sampling method based on the saliency map.

\subsubsection{Implementation Details}
\label{sec:4:experimental setup:implementation_details}

The proposed MB-RAICS is implemented with PyTorch~\cite{PyTorch} and the experiments are conducted on one Intel(R) Xeon(R) Platinum 8269CY CPU @ 2.50GHz and four NVIDIA GeForce RTX 3080 Ti GPUs. The single-stage rate-adaptive sampling model trains for 150 epochs, while the multi-stage rate-adaptive sampling model runs for 120 epochs. The learning rate starts at \(1 \times 10^{-4}\) for the initial 100 epochs and then decreases to \(1 \times 10^{-5}\) thereafter. The Adam optimizer is employed, with coefficients 0.9 and 0.999 used to compute running averages of the gradient and its square, respectively.
Other hyper-parameters are listed as follows: 
(\textbf{i}) The patch size, $B=32$.
(\textbf{ii}) The parameters for fitting the pair $(s_\text{r}, p_\text{s})$, $a=78.77,\ b=0.0444,\ s_{r;1}=0.01,\ p_{s;1}=0.005$.
(\textbf{iii}) The number of iterations at the decoder side, $L=5$.
(\textbf{iv}) The weight for the MSE loss, $\gamma=200$.

\subsection{Results and Analysis}
\label{sec:4:result and analysis}

\subsubsection{Comparison with State-of-the-Arts Methods}
\label{sec:4:result and analysis:comparison with state-of-the-arts methods}

Tab. \ref{tab:comparison with state-of-the-arts methods on five datasets} and Tab. \ref{tab:comparison with state-of-the-arts methods on two datasets} present the PSNR and SSIM results of MB-RAICS compared with 8 baselines across seven datasets at seven different sampling rates. We not only compare with the single-stage rate-adaptive version of CASNet but also with its two-stage version. In this two-stage version, the first stage employs uniform sampling, whereas the second stage uses the data from the first stage to infer a saliency map and implement rate-adaptive sampling. For labeling, the subscript "ss" is used with both CASNet and MB-RAICS to denote single-stage rate-adaptive sampling. The subscript "ms;$x$" is used to denote multi-stage rate-adaptive sampling, where $x$ indicates the number of sampling stages. When comparing MB-RAICS$_{\text{ss}}$ with uniform sampling methods such as CSNet, ISTA-Net$^+$, SCSNet, OPINE-Net, AMP-Net, COAST, and TransCS, MB-RAICS consistently demonstrates advantages across various datasets. For example, it exhibits an average gain of 1.93dB/0.0175 against OPINE-Net and 2.12dB/0.0208 against AMP-Net in PSNR/SSIM metrics. Compared to the single-stage rate-adaptive sampling version of CASNet, MB-RAICS$_{\text{ss}}$ also demonstrates an average gain of 0.85dB/0.0182. Moreover, MB-RAICS$_\text{ms;2}$ also outperforms uniform sampling methods. For example, compared to OPINE-Net, it achieves an average improvement of 1.38dB/0.0119. When compared to the two-stage rate-adaptive sampling version of CASNet, MB-RAICS$_\text{ms;2}$ also exhibits an average gain of 0.90dB/0.0141. Fig.~\ref{fig:visual comparison 1} and Fig.~\ref{fig:visual comparison 2} show the visualization results of different methods at sampling rates of 0.1 and 0.01, respectively. Notably, MB-RAICS outperforms other methods in reconstructing detailed textures and sharper edges.

%\input{Section/experiments_and_results_section/tables/multi-stage_table_7_datasets_two_methods_results}

\input{Section/experiments_and_results_section/figures/two-stage_figure_two_methods_visual_and_ratio_allocation_results_sampling_rate_0.04}

\paragraph{Comparison of Sampling Rate Allocation}

Fig.~\ref{fig:visual and rate allocation comparison 1} and Fig.~\ref{fig:visual and rate allocation comparison 2} respectively display the reconstruction and sampling rate allocation results of MB-RAICS and CASNet with two-stage rate-adaptive sampling and single-stage rate-adaptive sampling for an image from Set14 at a sampling rate of 0.04 and an image from Urban100 at a sampling rate of 0.25. In Fig.~\ref{fig:visual and rate allocation comparison 1}, it can be observed that the sampling rate allocation of MB-RAICS is relatively uniform over the foreground objects, while CASNet's allocation is more focused on the tree to the right of the foreground and the rooftop of the house in front. Comparatively, MB-RAICS's rate allocation may align more with human perception. In the region marked with a green box, where CASNet's sampling rate allocation tends to overlook, the reconstruction of MB-RAICS exhibits richer textures. In Fig.~\ref{fig:visual and rate allocation comparison 2}, MB-RAICS's rate allocation is relatively even across the foreground butterfly and the flower cluster on the left, whereas CASNet's allocation centers more on the butterfly. This could result in MB-RAICS's reconstructed details being more enriched in the flower cluster region enclosed by the green box.

\subsubsection{Ablation Studies}
\label{sec:4:result and analysis:ablation studies}
Tab.~\ref{tab:experiments of ablation studies of average PSNR across datasets} shows the experiments of ablation studies on average PSNR across 7 test datasets under 5 sampling rates. Specifically, Tab.\ref{tab:experiments of ablation studies of average PSNR across datasets} (1) represents our single-stage rate-adaptive sampling model. Tab.\ref{tab:experiments of ablation studies of average PSNR across datasets} (2)-(4) are variants based on Tab.\ref{tab:experiments of ablation studies of average PSNR across datasets} (1) that are designed for ablation studies. Tab.~\ref{tab:experiments of ablation studies of average PSNR across datasets} (5)-(8) represent our multi-stage rate-adaptive sampling models with different numbers of sampling stages.

\paragraph{Measurement-Bounds-based Rate-Adaptive Sampling v.s. Uniform Sampling}

We trained a variant that replaces the rate-adaptive sampling module in our method with uniform sampling. The results are presented in Tab.~\ref{tab:experiments of ablation studies of average PSNR across datasets} (2). Compared to the uniform sampling variant, our single-stage measurement-bounds-based rate-adaptive sampling model achieves an average improvement of 1.89 dB. This validates the effectiveness of our proposed method for allocating sampling rates.

\input{Section/experiments_and_results_section/figures/single-stage_figure_two_methods_visual_and_ratio_allocation_results_sampling_rate_0.25}

\input{Section/experiments_and_results_section/tables/single-stage_table_avg_PSNR_across_datasets_ablation_expriment_results}

\paragraph{Adaptive Overall Sparsity Ratio Based on Overall Sampling Rate v.s. Fixed Overall Sparsity Ratio}

In Sec.~\ref{sec:3:single-stage measurement-bounds-based rate-adaptive sampling:sparsity threshold}, we propose a method for determining the overall sparsity ratio based on the overall sampling rate. To test the effectiveness of this method, we trained a variant with a fixed overall sparsity ratio of 0.15, the results of which are recorded in Tab.~\ref{tab:experiments of ablation studies of average PSNR across datasets} (3). Compared to this variant, our method achieves an average improvement of 0.72~dB. This confirms the effectiveness of adjusting the overall sparsity ratio based on the overall sampling rate.

\paragraph{Impact of Decoder-Side Cross-Iteration Skip Connections}

We trained a variant without decoder-side cross-iteration skip connections, the results of which are shown in Tab.~\ref{tab:experiments of ablation studies of average PSNR across datasets} (4). Compared to this variant, our method achieves an average improvement of 0.09~dB. This confirms that decoder-side cross-iteration skip connections have a certain positive impact on performance.

\input{Section/experiments_and_results_section/figures/multi-stage_sampling_figure_ablation_experiment_mean_PSNR_results}

\paragraph{Study on the Number of Sampling Stages}

In the case of multi-stage rate-adaptive sampling, more sampling stages are expected to allocate the sampling rate more closely in proportion to the actual measurement bounds, thus potentially achieving higher performance. Tab.~\ref{tab:experiments of ablation studies of average PSNR across datasets} (5)-(8) presents the results of our multi-stage sampling models with 2, 5, 8, and 10 sampling stages, respectively. We find that increasing the number of sampling stages can boost performance; however, there is a diminishing return on this enhancement. Specifically, the model with 5 sampling stages is better than the 2-stage model by an average of 0.30 dB. However, going from 5 to 8 stages only gives a small improvement of 0.05 dB on average. Beyond 8 stages, the gains are minimal; upgrading to a 10-stage model results in only a slight improvement of 0.004 dB.


\paragraph{Impact of Optimizing Distribution Ratios on Sampling Rates}

In Sec.~\ref{sec:3:multi-stage rate-adaptive sampling strategy:sampling process:sampling in subsequent stages}, we introduce a distribution ratio optimization method, which is described in \eqref{eq:distribution ratio optimization}. To test the effectiveness of this method, we trained a variant without distribution ratio optimization. This variant uses the original distribution ratios \(\{p_i\}\) rather than the optimized \(\{q_i^{\star}\}\) for allocating the sampling rates. Fig.~\ref{fig:multi-stage sampling ablation studies} shows the average PSNR across seven test datasets and seven sampling rates for the proposed multi-stage rate-adaptive sampling method and this variant. Compared to the variant, our distribution ratio optimization method achieves an average improvement of 0.21~dB. This validates the effectiveness of the distribution ratio optimization method.

\input{Section/experiments_and_results_section/figures/single-stage_sampling_figure_robustness_experiment_rate_of_gain_change_results_against_change_in_test_images}

\subsubsection{Robustness Experiments for Measurement-Bounds-based Rate-Adaptive Sampling}

\paragraph{Robustness to Variations in Image Brightness, Scale, and Rotation angle}

To investigate the robustness of the proposed measurement-bound-based rate-adaptive sampling to variations in brightness, scale, and rotation angle, we adjusted these parameters in our test images. We set the brightness and scale of the original test images to $1$, and then proportionally adjusted the brightness and scale of the test images. We also set the rotation angle of the original test images to $0^\circ$ , and during testing, rotated the images around their center. Moreover, we conducted experiments on the saliency-based rate-adaptive sampling proposed in CASNet \cite{9854112} as a reference. To evaluate the variability of performance gains under different parameter settings, we introduce a metric called the rate of gain change (RGC):
\begin{equation}
	\text{RGC} = \frac{\text{performance improvement after change}}{\text{performance improvement before change}} - 1
\end{equation}
For example, when the brightness is $0.5$, the PSNR gain achieved by a model using rate-adaptive sampling compared to one using uniform sampling is $1.1$ dB. When the brightness is $1$, the PSNR gain of the model using rate-adaptive sampling is $1$ dB. Then the rate of gain change at brightness $0.5$ is $\frac{1.1}{1} - 1 = 10\%$.

Fig.~\ref{fig:single-stage sampling robustness experiments rate of gain change results against change in test images} shows the rate of gain change in average PSNR across seven test datasets and seven sampling rates under varying brightness, scale, and rotation angles for MB-RAICS with single-stage sampling and its variant with saliency-based rate-adaptive sampling, using the uniform sampling variant of MB-RAICS as the baseline. For variations in brightness, our method outperforms the saliency-based rate-adaptive variant, with RGC metrics being $12.96\%$ and $34.42\%$ higher at brightness levels of $0.7$ and $1.4$, respectively. The differences in RGC at other brightness levels are relatively smaller. In terms of scale and rotation angle variations, our method consistently outperforms this variant, with an average advantage of $65.12\%$ for scale changes and $32.35\%$ for rotation angle changes. This suggests that the measurement-bounds-based rate-adaptive sampling demonstrates relatively better robustness in terms of performance gains compared to the saliency-based rate-adaptive sampling when subject to variations in brightness, scale, and rotation angle.

\input{Section/experiments_and_results_section/figures/single-stage_sampling_figure_robustness_experiment_psnrs_against_different_decoders}

\paragraph{Robustness to Different Decoders}

Fig.~\ref{fig:single-stage sampling robustness experiments psnrs against different decoders} shows the average PSNR results of our single-stage measurement-bounds-based rate-adaptive sampling, single-stage saliency-based rate-adaptive sampling, and uniform sampling when combined with different decoders across six test datasets (excluding Urban100) and seven sampling rates. The Urban100 dataset was excluded because its relatively large image sizes caused the GPU memory requirements to surpass our current GPUs' capabilities when deploying the TransCS decoder. From the results, it is evident that our measurement-bounds-based rate-adaptive sampling method, in comparison with the uniform sampling combined with various decoders, shows a relatively stable improvement, exhibiting a performance increase with a standard deviation of $0.21$dB. On the other hand, the performance variability for saliency-based rate-adaptive sampling in relation to the uniform sampling has a standard deviation of $1.57$dB. Specifically, the performance of the saliency-based rate-adaptive sampling when combined with ISTA-Net$^{+}$ and OPINE-Net decoders appears less stable, registering performance declines of $3.62$dB and $0.07$dB, respectively, relative to the uniform sampling. These findings indicate that our measurement-bounds-based rate-adaptive sampling demonstrates better robustness to decoder variations than the saliency-based rate-adaptive sampling.







==> Section/experiments_and_results_section/tables/multi-stage_table_7_datasets_two_methods_results.tex <==
\begin{table*}
\centering
\caption{PSNR and SSIM comparisons for MB-RACS and CASNet with multi-stage rate-adaptive sampling on Set11, CBSD68, Set5, Set14, BSDS100, Urban100, and Kodak24 datasets at sampling rates of 0.01, 0.04, 0.1, 0.25, 0.3, 0.4, and 0.5. }
\label{tab:multi-stage-sampling-based comparison with CASNet on seven datasets}
\resizebox{\linewidth}{!}{
\begin{tabular}{c c c c c c c c c c c c c c c c}
\toprule
\multirow{2}{*}[-1em]{Dataset} & \multirow{2}{*}[-1em]{Method} & \multicolumn{14}{c}{Sampling Ratio} \\ \cmidrule(lr){3-16} 
& & \multicolumn{2}{c}{0.01} & \multicolumn{2}{c}{0.04} & \multicolumn{2}{c}{0.1} & \multicolumn{2}{c}{0.25} & \multicolumn{2}{c}{0.3} & \multicolumn{2}{c}{0.4} & \multicolumn{2}{c}{0.5} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16} & & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM & PSNR & SSIM \\
\midrule

  \specialrule{0em}{1pt}{1pt}
\midrule
\multirow{8}{*}[1.3em]{Set11} & CASNet$_\text{i;2}$ & 21.88 & 0.6012 & 26.66 & 0.7909 & 30.66 & 0.8806 & 35.46 & 0.9428 & 36.66 & 0.9524 & 38.71 & 0.9656 & 40.70 & 0.9750 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 22.30 & 0.6180 & 27.41 & 0.8134 & 31.52 & 0.8986 & 36.62 & 0.9544 & 37.81 & 0.9621 & 40.00 & 0.9725 & 41.83 & 0.9790 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 22.43 & 0.6225 & 27.56 & 0.8158 & 31.74 & 0.9011 & 36.89 & 0.9559 & 38.07 & 0.9628 & 40.09 & 0.9721 & 42.14 & 0.9792 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 22.52 & 0.6241 & 27.60 & 0.8174 & 31.79 & 0.9025 & 36.93 & 0.9557 & 38.11 & 0.9628 & 40.23 & 0.9726 & 42.21 & 0.9793 \\
 \midrule
 
\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[1.8em]{CBSD68} & CASNet$_\text{i;2}$ & 23.03 & 0.5491 & 26.00 & 0.6823 & 28.56 & 0.7892 & 32.50 & 0.8952 & 33.63 & 0.9147 & 35.82 & 0.9433 & 38.06 & 0.9628 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 23.37 & 0.5617 & 26.43 & 0.7005 & 29.20 & 0.8107 & 33.51 & 0.9144 & 34.72 & 0.9319 & 37.05 & 0.9558 & 39.38 & 0.9709 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 23.52 & 0.5651 & 26.65 & 0.7055 & 29.48 & 0.8159 & 33.89 & 0.9176 & 35.15 & 0.9344 & 37.58 & 0.9574 & 39.99 & 0.9723 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 23.53 & 0.5655 & 26.65 & 0.7058 & 29.49 & 0.8164 & 33.93 & 0.9182 & 35.20 & 0.9349 & 37.65 & 0.9578 & 40.08 & 0.9725 \\
 \midrule

\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[1.8em]{Set5} & CASNet$_\text{i;2}$ & 23.46 & 0.6580 & 28.73 & 0.8327 & 33.04 & 0.9082 & 37.65 & 0.9542 & 38.78 & 0.9614 & 40.89 & 0.9719 & 43.04 & 0.9796 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 23.83 & 0.6609 & 29.74 & 0.8524 & 33.73 & 0.9187 & 38.35 & 0.9594 & 39.58 & 0.9661 & 41.97 & 0.9756 & 44.20 & 0.9819 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 23.99 & 0.6744 & 29.89 & 0.8552 & 33.83 & 0.9204 & 38.60 & 0.9605 & 39.84 & 0.9669 & 42.19 & 0.9758 & 44.35 & 0.9822 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 23.99 & 0.6714 & 29.99 & 0.8570 & 33.1 & 0.9216 & 38.62 & 0.9607 & 39.85 & 0.9668 & 42.23 & 0.9758 & 44.43 & 0.9822 \\
 \midrule

\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[1.8em]{Set14} & CASNet$_\text{i;2}$ & 22.50 & 0.5612 & 26.18 & 0.7043 & 29.19 & 0.8108 & 33.56 & 0.9052 & 34.63 & 0.9209 & 36.68 & 0.9442 & 38.74 & 0.9604 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 22.86 & 0.5757 & 26.84 & 0.7252 & 30.21 & 0.8323 & 34.52 & 0.9189 & 35.63 & 0.9330 & 37.76 & 0.9524 & 39.67 & 0.9645 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 23.03 & 0.5793 & 27.04 & 0.7272 & 30.48 & 0.8351 & 34.74 & 0.9199 & 35.83 & 0.9334 & 37.90 & 0.9521 & 39.91 & 0.9645 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 23.08 & 0.5796 & 27.10 & 0.7289 & 30.51 & 0.8358 & 34.80 & 0.9201 & 35.93 & 0.9339 & 38.01 & 0.9524 & 39.95 & 0.9644 \\
 \midrule

\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[1.8em]{BSDS100} & CASNet$_\text{i;2}$ & 22.98 & 0.5335 & 25.80 & 0.6657 & 28.36 & 0.7764 & 32.27 & 0.8880 & 33.38 & 0.9085 & 35.56 & 0.9390 & 37.77 & 0.9597 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 23.29 & 0.5454 & 26.20 & 0.6827 & 28.91 & 0.7963 & 33.17 & 0.9063 & 34.37 & 0.9251 & 36.68 & 0.9512 & 38.99 & 0.9678 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 23.42 & 0.5482 & 26.41 & 0.6874 & 29.17 & 0.8011 & 33.51 & 0.9090 & 34.75 & 0.9272 & 37.15 & 0.9525 & 39.51 & 0.9690 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 23.43 & 0.5483 & 26.41 & 0.6876 & 29.18 & 0.8016 & 33.55 & 0.9097 & 34.79 & 0.9278 & 37.20 & 0.9528 & 39.59 & 0.9692 \\
 \midrule

\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[1.8em]{Urban100} & CASNet$_\text{i;2}$ & 20.15 & 0.5320 & 23.85 & 0.7154 & 27.14 & 0.8272 & 31.67 & 0.9157 & 32.84 & 0.9304 & 35.04 & 0.9519 & 37.19 & 0.9666 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 20.66 & 0.5565 & 24.68 & 0.7459 & 28.28 & 0.8556 & 33.10 & 0.9352 & 34.30 & 0.9472 & 36.48 & 0.9635 & 38.62 & 0.9743 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 20.83 & 0.5619 & 24.92 & 0.7511 & 28.59 & 0.8593 & 33.44 & 0.9367 & 34.66 & 0.9482 & 36.95 & 0.9641 & 39.17 & 0.9747 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 20.84 & 0.5617 & 24.91 & 0.7514 & 28.59 & 0.8598 & 33.47 & 0.9370 & 34.70 & 0.9484 & 37.01 & 0.9642 & 39.27 & 0.9748 \\
 \midrule

\specialrule{0em}{1pt}{1pt}
\midrule
\multirow{9}{*}[1.8em]{Kodak24} & CASNet$_\text{i;2}$ & 24.13 & 0.6009 & 27.21 & 0.7244 & 30.13 & 0.8191 & 34.55 & 0.9126 & 35.71 & 0.9291 & 37.91 & 0.9533 & 40.06 & 0.9692 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;2}$ & 24.57 & 0.6155 & 27.77 & 0.7444 & 30.88 & 0.8405 & 35.54 & 0.9276 & 36.79 & 0.9419 & 39.06 & 0.9611 & 41.19 & 0.9731 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;5}$ & 24.67 & 0.6186 & 28.05 & 0.7485 & 31.26 & 0.8444 & 35.93 & 0.9299 & 37.20 & 0.9436 & 39.52 & 0.9619 & 41.76 & 0.9737 \\ \cmidrule(l){2-16}
 & MB-RACS$_\text{i;8}$ & 24.68 & 0.6185 & 28.08 & 0.7501 & 31.27 & 0.8458 & 36.01 & 0.9306 & 37.26 & 0.9439 & 39.60 & 0.9621 & 41.86 & 0.9738 \\
 \midrule
 \specialrule{0em}{4pt}{1pt}
 \bottomrule
 \end{tabular}
} 
\end{table*}

==> Section/introduction_old.tex <==
\section{Introduction}\label{sec:introduction}
Compressed sensing (CS) has established a novel framework for sampling and reconstruction, complete with theoretical guarantees, which permits the remarkably precise reconstruction of sparse signals with considerably fewer measurements than stipulated by the Nyquist sampling theorem.
This mathematical theorem posits that, given a randomly formed measurement matrix $\boldsymbol{\Phi} \in \mathbb{R}^{m\times n}$ for any sparse signal $\textbf{\textit{x}}\in\mathbb{R}^n$, provided the number of measurements $m\geq Ck\log(n/k)$ - where $C$ is a constant and $k=\|\Psi \textbf{\textit{x}}\|_0$ represents the quantity of non-zero values in the sparse representation of $\textbf{\textit{x}}$ after a linear transformation - the original signal can be accurately reconstructed from the sampled signal $\textbf{\textit{y}}=\boldsymbol{\Phi} \textbf{\textit{x}}$. Crucially, when $k$ is small, a smaller number of measurements $m$ still allows for successful signal reconstruction.
This impressive capability has fueled the extensive application of CS across numerous disciplines, encompassing magnetic resonance imaging (MRI) \cite{4472246, https://doi.org/10.1002/mrm.21391}, computed tomography \cite{8271999}, wireless broadcast \cite{yin2016compressive, 6457441}, network measurement \cite{265057}, among others.

%传统的非深度的图像压缩感知方法。
Classical image CS approaches, termed optimization-based methods, frame the ill-posed linear inverse problem of CS reconstruction as an optimization problem based on image priors. The solution of these problems are then approximated using iterative methods. Notably, numerous papers have introduced reconstruction algorithms premised on diverse priors such as sparsity \cite{5414429}, local smoothness \cite{li2013efficient}, non-local self-similarity \cite{6341094}, and group-based sparsity \cite{6814320}. Nonetheless, the priors deployed in optimization-based methods do not wholly align with data traits, and the complexity required for iterative solutions is typically high.

%基于深度学习的图像压缩感知方法。
In recent years, numerous deep image CS methods have emerged, merging deep learning concepts with CS mechanisms, leading to enhanced reconstruction quality and speed. \cite{8765626} designed an end-to-end deep image CS structure, employing a data-driven strategy to guide the learning of measurement matrices and the reconstruction network. \cite{Zhang_2018_CVPR} proposed a deep unfolding method that converted an originally non-differentiable optimization method into an iterative network structure amenable to parameter updates through backpropagation. Integrating optimization-based method with data-driven understanding led to a significant enhancement in algorithm performance. Building on the deep unfolding concept, \cite{9298950} transformed the approximate message-passing (AMP) \cite{doi:10.1073/pnas.0909892106} into a network structure and utilized convolutional neural networks (CNN) to manage inter-block relationships, effectively alleviating block effects. \cite{9934025} focused on network structure design, introducing Transformers \cite{NIPS2017_3f5ee243} to the reconstruction network structure to model the long-distance dependencies between blocks.

%自适应与可扩展采用的深度图像压缩感知方法。
In addition to the learning of the measurement matrix and the design of the reconstruction network, there exists a range of research concerned with aspects such as model scalability and adaptive sampling ratio allocation. \cite{Shi_2019_CVPR} explored the scalability of the count of measurements, achieving coarse-grained scalability via hierarchical network structure design, and realizing fine-grained scalability through greedy algorithms, constructing a model that can adjust to varying sampling rates. \cite{9467810} offers a random projection augmentation strategy to facilitate a single model solution for the CS problem with any sampling matrix. \cite{5585813} proposes a compressed sampling scheme based on saliency information. By considering human visual attention, more perceptual resources are allocated to salient regions, thereby improving image reconstruction quality. \cite{9159912} utilizes a similar CS ratio allocation method and puts forward a multi-channel deep network structure. This allows image blocks with different sampling rates to be reconstructed by a unified model. \cite{9854112} puts forward a content-aware scalable deep CS network dubbed CASNet. It employs a data-driven saliency detector to generate saliency maps, then applies a block ratio aggregation strategy for adaptive sampling ratio allocation.

%我们的策略。
This study chiefly aims to develop an approach for adaptive allocation of sampling rates. Existing theoretical frameworks indicate that given a specific measurement matrix, the effective reconstruction of any sparse signal is possible provided the number of measurements surpasses the measurement bounds. Intrinsically, these bounds are associated with the sparsity of the block; a block with a higher degree of sparsity will have an elevated measurement bound, as stipulated by the formula discussed in the preceding paragraph. This inspires us to allocate sampling rates proportionally according to the measurement bounds across  different blocks. The successful application of our method depends on acquiring block sparsity information. In real-world instances where this data is inaccessible, we suggest a multi-stage rate-adaptive sampling approach. Under this method, the sampling process is broken down into several segments. Data from initial segments guides our prediction of measurement bounds, which in turn informs the allocation of sampling rates for the following segment. However, complete adherence to predicted measurement bounds in assigning sampling rates is not feasible due to the predetermined allocation in earlier steps. Consequently, we present a convex optimization algorithm as a partial solution to this issue. Utilizing both Newton's method and binary search, we identify the optimal solution for this optimization problem. Moreover, to ensure thorough relay of feature information during the forward phase, we incorporate cross-iteration skip connections within the decoder.

%分点总结我们的贡献点。
The contributions of this paper are as follows:

\begin{itemize}[leftmargin=1em]
\item We propose a measurement-bounds-based rate-adaptive image CS algorithm, wherein each block's sampling rate is proportionally aligned with its respective measurement bounds.

\item A multi-stage rate-adaptive sampling approach is presented as a solution for real-world situations where obtaining block sparsity information might be unattainable.

\item We develop cross-iteration skip connections at the decoding stage, which promotes efficient propagation of feature information over multiple iterations.

\item Experiments validate that MB-RAICS outperforms state-of-the-art approaches, with each component's functionality receiving empirical affirmation. The measurement-bounds-based rate-adaptive sampling's robustness against alterations in illumination, scale, and rotation angle has been effectively demonstrated as well.

\item Experiments validate that MB-RAICS outperforms state-of-the-art approaches, with each component's functionality and the robustness of measurement-bounds-based rate-adaptive sampling against alterations in illumination, scale, and rotation angle receiving empirical affirmation. 
\end{itemize}


==> Section/introduction_old_2.tex <==
\section{Introduction}\label{sec:introduction}
Compressed sensing (CS) has established a novel framework for sampling and reconstruction with theoretical guarantees, which permits the remarkably precise reconstruction of sparse signals with considerably fewer measurements than stipulated by the Nyquist sampling theorem.
This mathematical theorem posits that, given a randomly formed measurement matrix $\boldsymbol{\Phi} \in \mathbb{R}^{m\times n}$, for any sparse signal $\textbf{\textit{x}}\in\mathbb{R}^n$, provided the number of measurements $m\geq Ck\log(n/k)$ - where $C$ is a constant and $k=\|\Psi \textbf{\textit{x}}\|_0$ represents the quantity of non-zero values in the sparse representation of $\textbf{\textit{x}}$ after a linear transformation - the original signal can be accurately reconstructed from the sampled signal $\textbf{\textit{y}}=\boldsymbol{\Phi} \textbf{\textit{x}}$. For the signals encountered in practice, their $k$ is often small, and therefore the number of required measurements will be small as well. This impressive result has fueled the extensive application of CS across numerous disciplines, encompassing magnetic resonance imaging (MRI) \cite{4472246, https://doi.org/10.1002/mrm.21391}, computed tomography \cite{8271999}, wireless broadcast \cite{yin2016compressive, 6457441}, network measurement \cite{265057}, among others.

%传统的非深度的图像压缩感知方法。
Classical image CS approaches, termed optimization-based methods, frame the ill-posed linear inverse problem of CS reconstruction as an optimization problem based on image priors. The solution of these problems are then approximated using iterative methods. Notably, numerous papers have introduced reconstruction algorithms premised on diverse priors such as sparsity \cite{5414429}, local smoothness \cite{li2013efficient}, non-local self-similarity \cite{6341094}, and group-based sparsity \cite{6814320}. Nonetheless, the priors deployed in optimization-based methods do not wholly align with data traits, and the complexity required for iterative solutions is typically high.

%基于深度学习的图像压缩感知方法。
In recent years, numerous deep image CS methods have emerged, merging deep learning concepts with CS mechanisms, leading to enhanced reconstruction quality and speed. \cite{8765626} designed an end-to-end deep image CS structure, employing a data-driven strategy to guide the learning of measurement matrices and the reconstruction network. \cite{Zhang_2018_CVPR} proposed a deep unfolding method that converted an originally non-differentiable optimization method into an iterative network structure. Integrating optimization-based method with data-driven understanding led to a significant enhancement in algorithm performance. Building on the deep unfolding concept, \cite{9298950} transformed the approximate message-passing (AMP) \cite{doi:10.1073/pnas.0909892106} into a network structure. \cite{9934025} focused on network structure design, introducing Transformers \cite{NIPS2017_3f5ee243} to the reconstruction network structure to model the long-distance dependencies between blocks.

%自适应与可扩展采用的深度图像压缩感知方法。
In addition to the learning of the measurement matrix and the design of the reconstruction network, there exists a range of research concerned with aspects such as model scalability and adaptive sampling ratio allocation. \cite{Shi_2019_CVPR} explored the scalability of the count of measurements, achieving coarse-grained scalability via hierarchical network structure design, and realizing fine-grained scalability through greedy algorithms, constructing a model that can adjust to varying sampling rates. \cite{9467810} offers a random projection augmentation strategy to facilitate a single model solution for the CS problem with any sampling matrix. \cite{5585813} proposes a compressed sampling scheme based on saliency information. By considering human visual attention, more perceptual resources are allocated to salient regions, thereby improving image reconstruction quality. \cite{9159912} utilizes a similar CS ratio allocation method and puts forward a multi-channel deep network structure. \cite{9854112} puts forward a content-aware scalable deep CS network dubbed CASNet. It employs a data-driven saliency detector to generate saliency maps for adaptive sampling ratio allocation.

%我们的策略。
This study chiefly aims to develop an approach for adaptive allocation of sampling rates. 

Established theories show that effective sparse signal reconstruction is achievable when the number of measurements exceeds measurement bounds. This inspires us to allocate sampling rates proportionally according to the measurement bounds across different blocks. It is worth noting that the calculation of measurement bounds depends on the sparsity of the signal. For situations where block sparsity information can be acquired prior to sampling, we propose a single-stage measurement-bounds-based rate-adaptive sampling method. In real-world instances where this data is inaccessible, we suggest a multi-stage rate-adaptive sampling strategy. Under this strategy, the sampling process is broken down into several segments. Data from initial segments guides our prediction of measurement bounds, which further informs the allocation of sampling rates for the following segment. However, complete adherence to predicted measurement bounds in assigning sampling rates is not feasible because some of the sampling rates have already been allocated in previous sampling stages. Consequently, we present a convex optimization algorithm to optimize the allocation of sampling rates. Utilizing both Newton's method and the bisection method, we identify the optimal solution for this optimization problem. Moreover, to ensure thorough relay of feature information during the forward phase, we incorporate cross-iteration skip connections within the decoder.

%分点总结我们的贡献点。
The contributions of this paper are as follows:

\begin{itemize}[leftmargin=1em]
\item We propose a measurement-bounds-based rate-adaptive image CS algorithm, wherein each block's sampling rate is proportionally aligned with its respective measurement bounds.

\item A multi-stage rate-adaptive sampling approach is presented as a solution for real-world situations where obtaining block sparsity information might be unattainable.

\item We develop cross-iteration skip connections at the decoding stage, which promotes efficient propagation of feature information over multiple iterations.

\item Experiments validate that MB-RAICS outperforms state-of-the-art approaches, with each component's functionality receiving empirical affirmation. The robustness of measurement-bounds-based rate-adaptive sampling has been effectively demonstrated as well.
\end{itemize}


==> Section/proposed_method_old.tex <==
Subsequently, a DCT transformation is applied to each block, leading to the set $F_b=\{f_i\mid f_i=C(x_i), i=1,\ldots,\lceil\frac{H}{B}\rceil\lceil \frac{W}{B}\rceil\}$, where $C()$ represents the DCT transformation.

==> Section/proposed_method_subsection/draft.tex <==
The traditional CS measurement bounds theory offers a rigorously validated response to both inquiries. Classical CS theory primarily identifies a signal's complexity based on its sparsity within a specific domain. 
%This is logical; for instance, if the high-frequency coefficients of a block's discrete cosine transform (DCT) are of high magnitude, we perceive the block to contain intricate texture details. If these coefficients approach zero, the block is seen as more akin to a smooth surface, hence holding less information. 
Additionally, traditional CS theory validates that a faithful reconstruction is attainable when 
\begin{align}
    m>=Ck\log(n/k), \label{eq:measurement_bounds}
\end{align}
as mentioned in Sec.~\ref{sec:introduction}, where $C$ is a constant, $k$ is the sparsity of the signal, $n$ is the signal length, $m$ accounts for the number of measurements, and $Ck\log(n/k)$ is referred to as the measurement bounds. 


Using the measurement bounds theory as our foundation, in the following, we will introduce an engineered two-stage method to facilitate the implementation of the measurement-bound-based rate-adaptive sampling, with Fig.~\ref{fig:measurement-bounds-based_rate-adaptive_sampling_illustration} illustrating the associated sampling process.


This process aids in deriving the correlation between the sparsity threshold and the global sparsity ratio $p_s$:


Let's assume that $s_r$ represents the global sampling rate. As per \eqref{eq:measurement_bounds}, the indication is that a surge in sparsity would coincide with an increment in the number of measurements. Viewing this from another perspective, when the global sampling rate is predetermined and the global sparsity ratio is manipulable via the sparsity threshold, the global sparsity ratio is expected to exhibit a certain functional relationship with the global sampling rate. Intuitively, a boost in the global sampling rate should result in an upward trend in the global sparsity ratio. Our objective is to explore the correlation between these two metrics via experiments.


This is visually represented in the "Empirical Relationship" in Fig.~\ref{fig:s_r_p_s}, which illustrates the link between the $(s_r, p_s)$ pairs that we found to optimize model performance, where $s_r$ represents the overall sampling rate.


Thus, in setting the sparsity threshold, we initially identify the corresponding $p_s$ for a specified $s_r$ based on the fitted curve. Subsequently, we locate the corresponding $T$ as per \eqref{eq:overall_sparsity_ratio}, and given the limited search space and the lack of high-precision solution necessity, we employ an exhaustive search for the resolution.


Next, we concatenate the initial reconstructions of each block to form the entire image's initial reconstruction $\hat{\textit{\textbf{x}}}^0$. We then utilize the iterative decoder proposed in \cite{9854112}. Starting with $\hat{\textit{\textbf{x}}}^0$, we iterate $L$ times to obtain the reconstructed image.


Specifically, the decoder proposed in \cite{9854112} integrates gradient descent, adaptive sampling rate features concatenation, and a U-net architecture \cite{ronneberger2015u} for each iteration. The U-net is structured with three $2\times 2$ downsampling blocks, a central body block, and three $2\times 2$ upsampling blocks, represented as green, gray, and blue rectangles in the figure.

==> Section/proposed_method_subsection/multi-stage_rate-adaptive_sampling_strategy_old.tex <==
\subsection{Multi-Stage Rate-Adaptive Sampling Strategy}\label{sec:3:multi-stage rate-adaptive sampling strategy}

The aforementioned method assumes that we can access sparsity information of the signal prior before sampling. However, this isn't always feasible in certain practical scenarios. Take single-pixel imaging \cite{4472247}, for example, where we lack prior knowledge about the image being captured, making it challenging to deduce the level of sparsity in a given area. To overcome this, we introduce a multi-stage rate-adaptive sampling strategy, partitioning the sampling process into several stages. Leveraging information from previous samplings, we estimate the required allocation proportion. This estimation then informs the allocation of the sampling rate and the count of measurements for the succeeding sampling phase. Fig.~\ref{fig:multi-stage_rate-adaptive_sampling_strategy} illustrates the process of the multi-stage rate-adaptive sampling strategy.

To elaborate, let's assume we partition the sampling process into $N$ phases, each characterized by a roughly equivalent sampling rate of $s_r/N$, allowing for rounding deviations. In the initial phase, each block is sampled at an identical rate, given that we haven't yet gathered any information about the image. However, for the remaining $N-1$ phases, we predict the measurement bounds based on the previous sampled signals.

\subsubsection{Sampling in the First Stage}
We establish the sampling rate for the first  stage to be $s_r^1=s_r/N$. For the $i^{\text{th}}$ block, the count of measurements in this stage is given by $M_i^1=M^1=\floor{s_r^1B^2}$. We then proceed to sample the $i^{\text{th}}$ block by selecting the initial $M^1$ rows of $\textbf{\textit{A}}$:
\begin{align}
    \textbf{\textit{y}}_i^1 = \textbf{\textit{A}}_{1:M^1}\mathcal{V}(\textbf{\textit{x}}_i).
\end{align}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/multi-stage sampling strategy.pdf}
\caption{Illustration of the multi-stage rate-adaptive sampling strategy: the first sampling stage employs rate-fixed sampling, with subsequent sampling stages involving measurement bounds prediction, optimization of allocation ratio, measurements allocation, and rate-adaptive sampling.}
\label{fig:multi-stage_rate-adaptive_sampling_strategy}
\end{figure*}

\subsubsection{Sampling in Subsequent Stages}
\label{sec:3:multi-stage rate-adaptive sampling strategy:sampling in subsequent stages}
During the $t^{\text{th}}$ sampling phase, for $t>1$, the cumulative sampling rate for the first $t-1$ stages is given by $\sum_i\sum_{j=1}^{t-1}M_i^j/HW$. Upon entering the $t^{\text{th}}$ sampling phase, the desired cumulative sampling rate up until this point should be $ts_r/N$. Thus, the sampling rate specifically for the $t^{\text{th}}$ stage is set to $s_r^t=ts_r/N-\sum_i\sum_{j=1}^{t-1}M_i^j/HW$. Notably, by this stage, we already have the results of the initial $t-1$ samples for each block. Given this information, we designed a measurement bounds prediction network that uses these sampling results to predict the measurement bounds of these blocks:
\begin{align}
g_{\boldsymbol{\theta}_m}\left(\left[{\textbf{\textit{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{t-1}}^\transpose, 0, \ldots, 0\right]^\transpose\right)=\hat{m}_i^t.
\end{align}
The measurement bounds prediction network $g_{\boldsymbol{\theta}_m}$ consists of several CNN layers and residual blocks \cite{He_2016_CVPR}, where $\boldsymbol{\theta}_m$ represents the network parameters.  $\textbf{\textit{y}}_i^1, \ldots, \textbf{\textit{y}}_i^{t-1}$ represent the sampling signals obtained from the first $t-1$ sampling times. Since the length of the concatenated sampling signal can differ for each block, we pad zeros to the end of each concatenated sampling signal to ensure a consistent length of $B^2$. We compute the Kullback-Leibler (KL) divergence to measure the discrepancy when the predicted measurement bounds $\hat{m}_i^t$ are employed to approximate the actual measurement bounds $m_i$, both in terms of distribution ratios, and use this KL divergence for network training:
\begin{align}
    \mathcal{L}_{\text{KL}}=\frac{1}{(N-1)\frac{HW}{B^2}}\sum_{t=2}^N\sum_i-\frac{m_i}{\sum_im_i}\log\frac{\hat{m}_i^t}{\sum_i\hat{m}_i^t}. 
    \label{eq:KL loss for measurement bounds prediction network training}
\end{align}

\paragraph{Distribution Ratio Optimization}
Once we've obtained the predicted measurement bounds, we face a notable challenge: we want the proportion of the total measurement count allocated to the $i^{\text{th}}$ block at the $t^{\text{th}}$ stage to be $p_i=\frac{\hat{m}_i^t}{\sum_i\hat{m}_i^t}$. However, $\sum_i\sum_{j=1}^{t-1}M_i^j$ measurements have already been allocated to these blocks, a fact that cannot be altered. Our only recourse is to adjust the count of measurements related to the current sampling rate $s_r^t$, to make the overall allocation ratio converge towards $\{p_i\}$. 

To be specific, our desired allocation ratio is $\{p_i\}$, and the fixed allocation ratio for the $i^{\text{th}}$ block is $r_i=\frac{\sum_{j=1}^{t-1}M_i^j}{\sum_i\sum_{j=1}^{t-1}M_i^j}$. The proportion of the allocated sampling rate to the sum of the allocated and adjustable sampling rates for the current stage is $\beta=\frac{\sum_i\sum_{j=1}^{t-1}M_i^j/HW}{ts_r/N}$. The proportion of our adjustable sampling rate is $\alpha=1-\beta=\frac{s_r^t}{ts_r/N}$. Suppose the allocation ratio of the adjustable part is $\{q_i\}$. Therefore, after the $t^{\text{th}}$ sampling stage, the real allocation ratio is $\{\alpha q_i+\beta r_i\}$. We expect to adjust $\{q_i\}$ so that $\{\alpha q_i+\beta r_i\}$ is close to $\{p_i\}$ under the measurement of KL divergence. We also need to establish the upper and lower bounds of $q_i$. Clearly, the lower bound of $q_i$ is 0. Given that the number of measurements for the $i^{\text{th}}$ block must not exceed the length of its original signal, and considering that the count of measurements for the $i^{\text{th}}$ block at the $t^{\text{th}}$ sampling stage is approximately $q_is_r^tHW$ (accounting for a rounding error), we can derive the following relationship:
\begin{align}
    q_is_r^tHW + \sum_{j=1}^{t-1}M_i^j \leq B^2.
\end{align}
Therefore, we can obtain the upper bound of $q_i$, $a_i=\frac{B^2-\sum_{j=1}^{t-1}M_i^j}{s_r^tHW}$. Finally, we integrate the above considerations into a convex optimization problem:
\begin{equation}
\begin{aligned}
\argmin_{\{q_i\}} \quad  - & \sum_ip_i\log (\alpha q_i+\beta r_i) \\
\text{subject to} \quad & \sum_i q_i = 1, \\
                        & 0 \leq q_i \leq a_i \quad \text{for all} \quad i. 
\end{aligned}
\end{equation}
We employ the Karush-Kuhn-Tucker (KKT) conditions to resolve this issue, with the solution procedure detailed in Appendix~\ref{appendix:solution}.

\paragraph{Solving the Lagrange Multipliers}

Building on our earlier discussion, we have derived the closed-form solution of the convex optimization problem as: $q_i^{\star} = \min\left(\max\left(0, \frac{p_i}{\nu^{\star}} - \frac{\beta r_i}{\alpha}\right), a_i\right)$. The next step involves calculating the value of the Lagrange multiplier $\nu^{\star}$, which in turn will help us determine the solution for $q_i$. To simplify our notation, we substitute $\nu^\star$ with $\frac{1}{s^\star}$ (based on the conclusion in Appendix~\ref{appendix:solution} that $\nu^\star > 0$, we only consider cases where $s^\star > 0$). This leads us to rewrite the closed-form solution of the convex optimization problem as:
\begin{align}
q_i^{\star} = \min\left(\max\left(0, s^{\star}p_i - \frac{\beta r_i}{\alpha}\right), a_i\right).
\label{eq:distribution ratio optimization}
\end{align}
Define $Q_i(s) = \min\left(\max\left(0, s p_i- \frac{\beta r_i}{\alpha}\right), a_i\right)$, and let $Q(s) = \sum_{i=1}^n Q_i(s)$. Our problem is transformed into finding the solution for $Q(s) = 1$.

Before examining the function $Q(s)$, let us first define some symbols: $N_l(s)=\{i|Q_i(s)=0\}$, $N_m(s)=\{i|0<Q_i(s)<a_i\}$ and $N_u(s)=\{i|Q_i(s)=a_i\}$. With the help of these symbols, we obtain another representation of $Q(s)$:
\begin{align}
    Q(s) = \sum_{i=1}^n Q_i(s) &= \sum_{i\in N_m(s)}(sp_i - \frac{\beta r_i}{\alpha}) + \sum_{i\in N_u(s)}a_i.
\end{align}
The derivative of $Q(s)$ with respect to $s$ can be formulated as:
\begin{align}
    Q'(s) &= \sum_{i\in N_m(s)}p_i.
\end{align}
The function $Q(s)$ should be a piecewise linear monotonically increasing function with its domain being $(0, +\infty)$ and its range being $[0, \sum_{i=1}^n a_i]$. The boundary points of each linear segment correspond to those points $s$ that cause changes in $\{N_\text{J}(s) | \text{J} = l, m, u\}$. Fig.~\ref{fig:the approximate shape of Q(s)} shows the approximate shape of the $Q(s)$ function.
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/Qs.png}
    \caption{The approximate graphical representation of the function $Q(s)$.}
    \label{fig:the approximate shape of Q(s)}
\end{figure}

Next, our goal is to locate the root of $Q(s)=1$ utilizing Newton's method. The principle behind Newton's method is the presumption that the function behaves as locally linear at each iterative step, and it's under this presumption that we identify the root. Specifically, in the $t^{\text{th}}$ iteration, we have:
\begin{align}
    1&=(s^{(t+1)}-s^{(t)})Q'(s^{(t)})+Q(s^{(t)}).
\end{align}
By relocating $s^{(t+1)}$ to the left side of the equation and shifting the other terms to the right side, we obtain:
\begin{align}
    & s^{(t+1)} = \frac{1-Q(s^{(t)})}{Q'(s^{(t)})}+s^{(t)} \nonumber \\
    & =\frac{1-\sum_{i\in N_m(s^{(t)})}(s^{(t)}p_i-\frac{\beta r_i}{\alpha})-\sum_{i\in N_u(s^{(t)})}a_i}{\sum_{i\in N_m(s^{(t)})}p_i}+s^{(t)} \nonumber \\
    & =\frac{1+\sum_{i\in N_m(s^{(t)})}\frac{\beta r_i}{\alpha}-\sum_{i\in N_u(s^{(t)})}a_i}{\sum_{i\in N_m(s^{(t)})}p_i}. \label{eq:newton_iter}
\end{align}
In general, \(\sum_{i\in N_m(s^{(t)})}p_i > 0\) and \(1+\sum_{i\in N_m(s^{(t)})}\frac{\beta r_i}{\alpha}-\sum_{i\in N_u(s^{(t)})}a_i > 0\). If other cases occur, it is usually due to the initial value of \(s\) being set too small or too large. Empirically, setting \(s^{(0)} = \frac{\beta}{\alpha}\) can avoid these situations. We set the termination condition for the solution algorithm as $\{N_\text{J}(s^{(t)}) | \text{J} = l, m, u\}$ being entirely equal to $\{N_\text{J}(s^{(t+1)}) | \text{J} = l, m, u\}$, that is, $s^{(t)}$ and $s^{(t+1)}$ are in the same linear function segment. In this case, we can deduce that \(s^{(t+1)}\) is the root of $Q(s) = 1$:
\begin{equation}
\begin{aligned}
    Q(s^{(t+1)}) & = \sum_{i\in N_m(s^{(t+1)})}(s^{(t+1)}p_i - \frac{\beta r_i}{\alpha}) + \sum_{i\in N_u(s^{(t+1)})}a_i \\
    & = \sum_{i\in N_m(s^{(t)})}(s^{(t+1)}p_i - \frac{\beta r_i}{\alpha}) + \sum_{i\in N_u(s^{(t)})}a_i \\
    & \stackrel{\text{According to \eqref{eq:newton_iter}}}{=}1. \nonumber
\end{aligned}
\end{equation}

Subsequently, we wish to consider the convergence issue of this Newton's method. The difficulty in directly referencing previous methods of proving the convergence of Newton's method is that the general Newton's method deals with smooth functions, and considers the convergence speed of the error upper bound as $t$ increases. However, in this specific scenario, during the Newton's iteration process, $s^{(t)}$ will fall into different linear segments, until $s^{(t)}$ falls into the linear segment identical to the root (as stated above, once we find the linear segment where the root is located, we can obtain the root through a single application of Newton's method). From this perspective, this problem is concerned with finding the root's linear segment from all possible linear segments, rather than focusing on the convergence speed of the error in the solution. Consequently, we are currently seeking to propose a fallback plan for when Newton's method fails to converge, ensuring that we eventually identify the linear segment hosting the root, instead of focusing on Newton's method's convergence rate.

To manage scenarios where Newton's method fails to converge, we first present Lemma \ref{lemma:inequality relationship} in Appendix~\ref{appendix:lemma}. This lemma allows us to understand the interval in which $s^\star$ is located and assists us further narrow down this interval. Specifically, we can determine the upper and lower bounds of $s^\star$ by comparing the relationship between $s^{(t)}$ and $s^{(t+1)}$. For example, if $s^{(t)} < s^{(t+1)}$, compare $s^{(t)}$ with the existing lower bound. If $s^{(t)}$ is greater than the current lower bound, set the lower bound to $s^{(t)}$.

\input{Section/proposed_method_subsection/newton_and_bisection_algorithm}

Next, we can assess the convergence at each stage of Newton's method by using predetermined upper and lower bounds. If a particular step doesn't converge, meaning it surpasses the upper or lower bound, we can utilize the bisection method to replace the result of that step by calculating the average of the lower and upper bounds. Even if all steps in Newton's method fail to converge, we can still use Lemma \ref{lemma:inequality relationship} to ascertain whether the root is smaller or larger than our current result. This, in turn, helps define the search interval for the bisection method, guiding the entire process to locate the root within the line segment via bisection method instead of Newton's method. We have developed Algorithm \ref{alg:find root with newton's method and bisection method} based on this methodology. Here, the function $\chi_\textbf{\textit{b}}(\bm{\omega}):\mathbf{R}^n \rightarrow \mathbf{R}^n$($\textbf{\textit{b}}\in \mathbf{R}^n$) is specified as:
\begin{align}
\chi_\textbf{\textit{b}}(\bm{\omega})_i= \begin{cases} 1 & \text{if } \omega_i=b_i \\ 0  & \text{if } \omega_i\neq b_i
\end{cases}
\end{align}

\paragraph{Distribution of Measurements}

Once we have determined the allocation ratio $\{q_i^\star\}$, we can allocate the sampling rate and the number of measurements to the $i^\text{th}$ block based on this ratio:
\begin{align}
    s_i^t & = \alpha q_i^{\star}s_r^t\frac{HW}{B^2},\\
    M_i^t & = \round{s_i^tB^2}.
\end{align}
Here, $\alpha$ plays a similar role as in \eqref{eq:distribute sampling rate}, its primary function being to align the actual sampling rate closely with the desired one. Next, we extract rows $\sum_{j=1}^{t-1}M_i^j+1$ through $\sum_{j=1}^{t}M_i^j$ from measurement matrix $\textit{\textbf{A}}$ to sample the $i^\text{th}$ block:
\begin{align}
    \textit{\textbf{y}}_i^t = \textit{\textbf{A}}_{\sum_{j=1}^{t-1}M_i^j+1:\sum_{j=1}^{t}M_i^j}\mathcal{V}(\textit{\textit{x}}_i).
\end{align}
After completing $N$ steps of sampling, we obtained the total number of measurements  as well as the final sampling result for the $i^{\text{th}}$ block:
\begin{align}
    M_i & = \sum_{j=1}^{N}M_i^j, \\
    \textit{\textbf{y}}_i & = \left[{\textit{\textbf{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{N}}^\transpose\right]^\transpose.
\end{align}


==> Section/proposed_method_subsection/multi-stage_rate-adaptive_sampling_strategy_old3.tex <==
\subsection{Multi-Stage Rate-Adaptive Sampling Strategy}\label{sec:3:multi-stage rate-adaptive sampling strategy}

The aforementioned method assumes that we can access sparsity information of the signal prior before sampling. However, this is not always feasible in certain practical applications. Taking single-pixel imaging \cite{4472247} as an example, if we consider photography as a sampling process, we cannot obtain information about the original image through other methods before sampling. To overcome this, we introduce a multi-stage rate-adaptive sampling strategy, partitioning the sampling process into several stages. Leveraging information from previous samplings, we estimate the measurement bounds for each block. This estimation then informs the allocation of the sampling rate and the count of measurements for the succeeding sampling stage. Fig.~\ref{fig:multi-stage_rate-adaptive_sampling_strategy} illustrates the process of the multi-stage rate-adaptive sampling strategy.

\subsubsection{Sampling Process}
To elaborate, assume that we partition the sampling process into $N$ stages, where each stage has an approximate sampling rate of $s_\text{r}/N$, allowing for rounding deviations.
In the first stage, each block is sampled at an identical rate, given that we haven't yet gathered any information about the image. For the remaining $N-1$ stages, we predict the measurement bounds based on the previous sampled signals.

\paragraph{Sampling in the First Stage}
We set the sampling rate for the first stage $s_\text{r}^1=s_\text{r}/N$. For the $i^{\text{th}}$ block, the count of measurements in this stage is given by $M_i^1=M^1=\floor{s_\text{r}^1B^2}$. We then proceed to sample the $i^{\text{th}}$ block using the initial $M^1$ rows of $\textbf{\textit{A}}$:
\begin{align}
    \textbf{\textit{y}}_i^1 = \textbf{\textit{A}}_{1:M^1}\mathcal{V}(\textbf{\textit{x}}_i).
\end{align}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/multi-stage sampling strategy.pdf}
\caption{Illustration of the multi-stage rate-adaptive sampling strategy: the first sampling stage employs rate-fixed sampling, with subsequent sampling stages involving measurement bounds prediction, optimization of allocation ratio, measurements allocation, and rate-adaptive sampling.}
\label{fig:multi-stage_rate-adaptive_sampling_strategy}
\end{figure*}

\paragraph{Sampling in Subsequent Stages}
\label{sec:3:multi-stage rate-adaptive sampling strategy:sampling process:sampling in subsequent stages}
Here, we are concerned with the sampling rate and measurements allocation for the $t^{\text{th}}$ (where $t > 1$) sampling stage. The actual 
cumulative sampling rate for the first $t-1$ stages is given by $\sum_i\sum_{j=1}^{t-1}M_i^j/HW$, where $M_i^j$ represents the actual number of measurements allocated to the $i^{\text{th}}$ block during the $j^{\text{th}}$ stage. Moreover, the expected 
cumulative sampling rate up to the $t^{\text{th}}$ sampling stage is set to $ts_\text{r}/N$. Thus, the expected sampling rate specifically for the $t^{\text{th}}$ stage $s_\text{r}^t=ts_\text{r}/N-\sum_i\sum_{j=1}^{t-1}M_i^j/HW$. Notably, by this stage, we already have the sampling results of the initial $t-1$ stages for each block. Therefore, we designed a measurement bounds prediction network that uses these sampling results to predict the measurement bounds of these blocks:
\begin{align}
g_{\boldsymbol{\theta}_m}\left(\left[{\textbf{\textit{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{t-1}}^\transpose, 0, \ldots, 0\right]^\transpose\right)=\hat{m}_i^t.
\end{align}
The measurement bounds prediction network $g_{\boldsymbol{\theta}_m}$ consists of several CNN layers and residual blocks \cite{He_2016_CVPR}, where $\boldsymbol{\theta}_m$ represents the network parameters.  $\textbf{\textit{y}}_i^1, \ldots, \textbf{\textit{y}}_i^{t-1}$ represent the sampling signals obtained from the first $t-1$ sampling stages for the $i^{\text{th}}$ block. Since the length of the concatenated sampling signal is likely to differ for each block, we pad zeros to the end of each concatenated sampling signal to ensure a consistent length of $B^2$. We compute the Kullback-Leibler (KL) Divergence-based loss to measure the discrepancy when the predicted measurement bounds $\hat{m}_i^t$ are employed to approximate the actual measurement bounds $m_i$, both in terms of distribution ratios, and use this KL divergence-based loss for network training:
\begin{align}
    \mathcal{L}_{\text{KL}}=\frac{1}{(N-1)\frac{HW}{B^2}}\sum_{t=2}^N\sum_i-\frac{m_i}{\sum_im_i}\log\frac{\hat{m}_i^t}{\sum_i\hat{m}_i^t}, 
    \label{eq:KL loss for measurement bounds prediction network training}
\end{align}
where the normalization factor of $\frac{1}{(N-1)\frac{HW}{B^2}}$ is chosen to average the loss over all sampling stages that have the step of predicting measurement bounds and over all blocks.

Upon we obtain the predicted measurement bounds, we set the expected proportion of measurements allocated to the $i^{\text{th}}$ block after the $t^{\text{th}}$ stage as $p_i^t = \frac{\hat{m}_i^t}{\sum_i \hat{m}_i^t}$. However, the expected proportion is likely not achievable due to the fixed allocation ratios in the first $t-1$ stages. Therefore, we can only adjust the allocation ratio for the current $t^{\text{th}}$ stage to make the actual cumulative allocation ratio over the first $t$ stages approximate the expected one. Sec. \ref{sec:3:multi-stage rate-adaptive sampling strategy:subproblem of distribution ratio optimization} describes the specific distribution ratio optimization method for allocating the sampling rate for the current $t^{\text{th}}$ stage. We define the allocation ratio of the $i^{\text{th}}$ block, optimized using the aforementioned method, as ${q_i^t}^{\star}$.

Once we determine the optimized allocation ratio, we can allocate the sampling rate and the number of measurements to the $i^\text{th}$ block based on this allocation ratio:
\begin{align}
    s_i^t & = \eta {q_i^t}^{\star}s_\text{r}^t\frac{HW}{B^2},\\
    M_i^t & = \round{s_i^tB^2}.
\end{align}
Here, $\eta$ plays a similar role as in \eqref{eq:distribute sampling rate}, its primary function being to align the actual sampling rate closely with the desired one. Next, we extract rows $\sum_{j=1}^{t-1}M_i^j+1$ through $\sum_{j=1}^{t}M_i^j$ from measurement matrix $\textit{\textbf{A}}$ to sample the $i^\text{th}$ block:
\begin{align}
    \textit{\textbf{y}}_i^t = \textit{\textbf{A}}_{\sum_{j=1}^{t-1}M_i^j+1:\sum_{j=1}^{t}M_i^j}\mathcal{V}(\textit{\textit{x}}_i).
\end{align}
After completing $N$ stages of sampling, we obtained the total number of measurements  as well as the final sampling result for the $i^{\text{th}}$ block:
\begin{align}
    M_i & = \sum_{j=1}^{N}M_i^j, \\
    \textit{\textbf{y}}_i & = \left[{\textit{\textbf{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{N}}^\transpose\right]^\transpose.
\end{align}

\subsubsection{Subproblem of Distribution Ratio Optimization}
\label{sec:3:multi-stage rate-adaptive sampling strategy:subproblem of distribution ratio optimization}

\paragraph{Problem Description}
In the following, we will define some symbols and describe the distribution ratio optimization problem as a convex optimization problem. The proportion of measurements yet to be allocated in the current $t^{\text{th}}$ stage and the proportion of measurements allocated in the first $t-1$ stages, with respect to the total number of allocatable measurements in the first $t$ stages, are given by $\alpha^t = \frac{s_\text{r}^t}{ts_\text{r}/N}$ and $ \beta^t = 1 - \alpha^t = \frac{\sum_i\sum_{j=1}^{t-1}M_i^j/HW}{ts_\text{r}/N}$, respectively. The fixed allocation ratio for the $i^{\text{th}}$ block is $r_i^t=\frac{\sum_{j=1}^{t-1}M_i^j}{\sum_i\sum_{j=1}^{t-1}M_i^j}$. Suppose the allocation ratio to be determined in the $t^{\text{th}}$ stage is $\{q_i^t\}$. Therefore, after the $t^{\text{th}}$ sampling stage, the actual allocation ratio is $\{\alpha^t q_i^t+\beta^t r_i^t\}$. Fig.~\ref{fig:distribution ratio optimization toy example} provides a toy example depicting $r_i^t$, $q_i^t$, $\beta^t$, and $\alpha^t$. Our objective is to adjust $\{q_i^t\}$ so that $\{\alpha^t q_i^t+\beta^t r_i^t\}$ is close to $\{p_i^t\}$ under the measurement of KL divergence-based object function. Additionally, $q_i^t$ is subject to upper and lower bounds. Clearly, the lower bound of $q_i^t$ is 0. Moreover, given that the number of measurements for the $i^{\text{th}}$ block must not exceed the length of its original signal, and considering that the count of measurements for the $i^{\text{th}}$ block at the $t^{\text{th}}$ sampling stage is approximately $q_i^ts_\text{r}^tHW$ (accounting for a rounding error), we can derive the following relationship:
\begin{align}
    q_i^ts_\text{r}^tHW + \sum_{j=1}^{t-1}M_i^j \leq B^2.
\end{align}
Therefore, we can obtain the upper bound of $q_i^t$, $a_i^t=\frac{B^2-\sum_{j=1}^{t-1}M_i^j}{s_\text{r}^tHW}$. Finally, we integrate the above considerations into a convex optimization problem:
\begin{equation}
\begin{aligned}
\argmin_{\{q_i^t\}} \quad  - & \sum_ip_i^t\log (\alpha^t q_i^t+\beta^t r_i^t) \\
\text{subject to} \quad & \sum_i q_i^t = 1, \\
                        & 0 \leq q_i^t \leq a_i^t \quad \text{for all} \quad i. 
\label{eq:allocation ratio optimization problem}                 
\end{aligned}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/distribution ratio optimization example.pdf}
\caption{A toy example of $r_i^t$, $q_i^t$, $\beta^t$, and $\alpha^t$.}
\label{fig:distribution ratio optimization toy example}
\end{figure}

\paragraph{Obtaining the Implicit Solution of the Optimization Problem Using the Lagrangian Multiplier  Method}

We employ the Karush-Kuhn-Tucker (KKT) conditions based on the Lagrange multiplier method to resolve this issue, yielding an implicit solution. The detailed procedure is provided in Appendix~A.

\paragraph{Solving for the Lagrange Multiplier to Obtain Explicit Solution}
We first frame the solution of the Lagrange multiplier as the problem of finding the root of a function. Building on our earlier discussion, we have derived the closed-form solution of the convex optimization problem as: ${q_i^t}^{\star} = \min\left(\max\left(\frac{p_i^t}{\nu^{\star}} - \frac{\beta^t r_i^t}{\alpha^t}, 0\right), a_i^t\right)$. The next step is to identify the value of the Lagrange multiplier $\nu^{\star}$ in order to determine the solution for ${q_i^t}^{\star}$. To simplify our notation, we substitute $\nu^\star$ with $\frac{1}{\mu^\star}$ (based on the conclusion in Appendix~A that $\nu^\star > 0$, we only consider cases where $\mu^\star > 0$). This leads us to rewrite the closed-form solution of the convex optimization problem as:
\begin{align}
{q_i^t}^{\star} = \min\left(\max\left(\mu^{\star}p_i^t - \frac{\beta^t r_i^t}{\alpha^t}, 0\right), a_i^t\right).
\label{eq:distribution ratio optimization}
\end{align}
Define $Q_i^t(\mu) = \min\left(\max\left(\mu p_i^t- \frac{\beta^t r_i^t}{\alpha^t}, 0\right), a_i^t\right)$, and let $Q^t(\mu) = \sum_i Q_i^t(\mu)$. Based on the constraint condition in \eqref{eq:allocation ratio optimization problem} that the sum of the allocation ratios should be equal to 1, our problem is transformed into finding $\mu$ that satisfies $Q^t(\mu) = 1$.

Before examining the function $Q^t(\mu)$, let us first define some notation: $N_\text{l}^t(\mu)=\{i|Q_i^t(\mu)=0\}$, $N_\text{c}^t(\mu)=\{i|0<Q_i^t(\mu)<a_i^t\}$ and $N_\text{u}^t(\mu)=\{i|Q_i^t(\mu)=a_i^t\}$. With the help of this notation, we obtain another representation of $Q^t(\mu)$:
\begin{align}
    Q^t(\mu) = \sum_i Q_i^t(\mu) &= \sum_{i\in N_\text{c}^t(\mu)}(\mu p_i^t - \frac{\beta^t r_i^t}{\alpha^t}) + \sum_{i\in N_\text{u}^t(\mu)}a_i^t.
\end{align}
The derivative of $Q^t(\mu)$ with respect to $\mu$ can be formulated as:
\begin{align}
    {Q^t}'(\mu) &= \sum_{i\in N_\text{c}^t(\mu)}p_i^t.
\end{align}
The function $Q^t(\mu)$ should be a piecewise linear monotonically increasing function with its domain being $(0, +\infty)$ and its range being $[0, \sum_{i=1}^n a_i^t]$. The boundary points of each linear segment correspond to those points $\mu$ that cause changes in $\{N_\text{J}(\mu) | \text{J} = \text{l}, \text{c}, \text{u}\}$. Fig.~\ref{fig:the approximate shape of Q(mu)} shows the approximate shape of the $Q^t(\mu)$ function.
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/Qmu.png}
    \caption{The approximate graphical representation of the function $Q^t(\mu)$.}
    \label{fig:the approximate shape of Q(mu)}
\end{figure}

%总的求根方法的描述
Next, we combine Newton's method with the bisection method to solve for the root of $Q^t(\mu) = 1$, ensuring efficient computation while guaranteeing convergence. Initially, we solve iteratively using Newton's method. If convergence is not achieved, we use the bisection method to ensure that the iterative solution remains within the known upper and lower bounds of the root.

\input{Section/proposed_method_subsection/newton_and_bisection_algorithm}

Specifically, the principle behind Newton's method is that during each iteration, it approximates the function as being locally linear around the current estimate and subsequently updates the root approximation based on this linear assumption. In the $\tau^{\text{th}}$ iteration, we have:
\begin{align}
    1&=(\mu^{(\tau+1)}-\mu^{(\tau)}){Q^t}'(\mu^{(\tau)})+Q^t(\mu^{(\tau)}),
\end{align}
where $\mu^{(\tau)}$ is the result of the $\tau^{\text{th}}$ iteration of Newton's method. By relocating $\mu^{(\tau+1)}$ to the left side of the equation and shifting the other terms to the right side, we obtain:
\begin{align}
    & \mu^{(\tau+1)} = \frac{1-Q^t(\mu^{(\tau)})}{{Q^t}'(\mu^{(\tau)})}+\mu^{(\tau)} \nonumber \\
    & =\frac{1-\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}(\mu^{(\tau)}p_i^t-\frac{\beta^t r_i^t}{\alpha^t})-\sum_{i\in N_\text{u}^t(\mu^{(\tau)})}a_i^t}{\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}p_i^t}+\mu^{(\tau)} \nonumber \\
    & =\frac{1+\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}\frac{\beta^t r_i^t}{\alpha^t}-\sum_{i\in N_\text{u}^t(\mu^{(\tau)})}a_i^t}{\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}p_i^t}. \label{eq:newton_iter}
\end{align}
In general, both the numerator and the denominator in the last expression of \eqref{eq:newton_iter} are greater than zero, unless the initial value for Newton's method is set too small or too large. Empirically, setting $\mu^{(0)} = \frac{\beta^t}{\alpha^t}$ ensures both are positive. We set the termination condition as $\{N_\text{J}^t(\mu^{(\tau)}) | \text{J} = \text{l}, \text{c}, \text{u}\}$ being entirely equal to $\{N_\text{J}^t(\mu^{(\tau+1)}) | \text{J} = \text{l}, \text{c}, \text{u}\}$, that is, $\mu^{(\tau)}$ and $\mu^{(\tau+1)}$ are in the same linear function segment. In this case, we can deduce that $\mu^{(\tau+1)}$ is the root of $Q^t(\mu) = 1$:
\begin{equation}
\begin{aligned}
    Q^t(\mu^{(\tau+1)}) & = \sum_{i\in N_\text{c}^t(\mu^{(\tau+1)})}(\mu^{(\tau+1)}p_i^t - \frac{\beta^t r_i^t}{\alpha^t}) + \sum_{i\in N_\text{u}^t(\mu^{(\tau+1)})}a_i^t \\
    & = \sum_{i\in N_\text{c}^t(\mu^{(\tau)})}(\mu^{(\tau+1)}p_i^t - \frac{\beta^t r_i^t}{\alpha^t}) + \sum_{i\in N_\text{u}^t(\mu^{(\tau)})}a_i^t \\
    & \stackrel{\text{According to \eqref{eq:newton_iter}}}{=}1. \nonumber
\end{aligned}
\end{equation}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/cross-iteration skip connections v2.pdf}
\caption{Illustration of the cross-iteration skip connections: we add the features output from the three upsampling blocks and the body block of the U-net in ${l-1}^\text{th}$ iteration to the features in the three downsampling blocks and the body block in the U-net of ${l}^\text{th}$ iteration.}
\label{fig:cross-iteration_skip_connection}
\end{figure}

Subsequently, we wish to consider the convergence issue of Newton's method under discussion. The difficulty in directly referencing previous methods of proving the convergence of Newton's method is that the general Newton's method deals with smooth functions, and considers the convergence speed of the error upper bound as $\tau$ increases. However, in this specific scenario, during the Newton's iteration process, $\mu^{(\tau)}$ will fall into different linear segments, until $\mu^{(\tau)}$ falls into the linear segment identical to the root (as stated above, once we find the linear segment where the root is located, we can obtain the root through one iteration of Newton's method). From this perspective, this problem is concerned with finding the root's linear segment from all possible linear segments, rather than focusing on the convergence speed of the error in the solution. 

Consequently, we are currently seeking to propose a fallback plan for when Newton's method fails to converge, ensuring that we eventually identify the linear segment hosting the root. We first present Lemma~B.1 in Appendix~B. This lemma allows us to understand the interval in which $\mu^\star$ is located and assists us further narrow down this interval. Specifically, we can determine the upper and lower bounds of $\mu^\star$ by comparing the relationship between $\mu^{(\tau)}$ and $\mu^{(\tau+1)}$. For example, if $\mu^{(\tau)} < \mu^{(\tau+1)}$, based on Lemma~B.1, we can deduce that $\mu^{(\tau)} < \mu^{\star}$. Then, compare $\mu^{(\tau)}$ with the existing lower bound; if $\mu^{(\tau)}$ is greater than the current lower bound, update the lower bound to $\mu^{(\tau)}$.

\input{Section/experiments_and_results_section/tables/single-stage_table_5_datasets_different_methods_results}
\input{Section/experiments_and_results_section/tables/single-stage_table_2_datasets_different_methods_results}

Next, we can assess the convergence at each iteration of Newton's method by using the upper and lower bounds obtained from Lemma~B.1. 
If the result of a particular iteration surpasses the upper or lower bound, we consider that this iteration has not converged. Therefore, we utilize the bisection method to replace the result of this iteration by the average of the lower and upper bounds. Even if all iterations in Newton's method fail to converge, we can still use Lemma~B.1 to ascertain whether the root is smaller or larger than our current result. This helps define the bisection method's search interval, guiding the overall process to locate the linear segment where the root lies via bisection method instead of Newton's method. We have developed Algorithm \ref{alg:find root with newton's method and bisection method} based on this methodology. For the sake of convenient notation, we have removed the superscript $t$ that indicates the stage number. Additionally, the function $\chi_\textbf{\textit{b}}(\bm{\omega}):\mathbb{R}^{\frac{HW}{B^2}} \rightarrow \mathbb{R}^{\frac{HW}{B^2}}$($\textbf{\textit{b}}\in \mathbb{R}^{\frac{HW}{B^2}}$) is specified as:
\begin{align}
\chi_\textbf{\textit{b}}(\bm{\omega})_i= \begin{cases} 1 & \text{if } \omega_i=b_i \\ 0  & \text{if } \omega_i\neq b_i
\end{cases}
\end{align}

==> Section/proposed_method_subsection/multi-stage_rate-adaptive_sampling_strategy_old_2_backup.tex <==
\subsection{Multi-Stage Rate-Adaptive Sampling Strategy}\label{sec:3:multi-stage rate-adaptive sampling strategy}

The aforementioned method assumes that we can access sparsity information of the signal prior before sampling. However, this is not always feasible in certain practical applications. Taking single-pixel imaging \cite{4472247} as an example, if we consider photography as a sampling process, we cannot obtain information about the original image through other methods before sampling. To overcome this, we introduce a multi-stage rate-adaptive sampling strategy, partitioning the sampling process into several stages. Leveraging information from previous samplings, we estimate the measurement bounds for each block. This estimation then informs the allocation of the sampling rate and the count of measurements for the succeeding sampling stage. Fig.~\ref{fig:multi-stage_rate-adaptive_sampling_strategy} illustrates the process of the multi-stage rate-adaptive sampling strategy.

\subsubsection{Sampling Process}
To elaborate, assume that we partition the sampling process into $N$ stages, where each stage has an approximate sampling rate of $s_\text{r}/N$, allowing for rounding deviations.
In the first stage, each block is sampled at an identical rate, given that we haven't yet gathered any information about the image. For the remaining $N-1$ stages, we predict the measurement bounds based on the previous sampled signals.

\paragraph{Sampling in the First Stage}
We set the sampling rate for the first stage $s_\text{r}^1=s_\text{r}/N$. For the $i^{\text{th}}$ block, the count of measurements in this stage is given by $M_i^1=M^1=\floor{s_\text{r}^1B^2}$. We then proceed to sample the $i^{\text{th}}$ block using the initial $M^1$ rows of $\textbf{\textit{A}}$:
\begin{align}
    \textbf{\textit{y}}_i^1 = \textbf{\textit{A}}_{1:M^1}\mathcal{V}(\textbf{\textit{x}}_i).
\end{align}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{Figures/multi-stage sampling strategy.pdf}
\caption{Illustration of the multi-stage rate-adaptive sampling strategy: the first sampling stage employs rate-fixed sampling, with subsequent sampling stages involving measurement bounds prediction, optimization of allocation ratio, measurements allocation, and rate-adaptive sampling.}
\label{fig:multi-stage_rate-adaptive_sampling_strategy}
\end{figure*}

\paragraph{Sampling in Subsequent Stages}
\label{sec:3:multi-stage rate-adaptive sampling strategy:sampling in subsequent stages}
Here, we are concerned with the sampling rate and measurements allocation for the $t^{\text{th}}$ (where $t > 1$) sampling stage. The actual 
cumulative sampling rate for the first $t-1$ stages is given by $\sum_i\sum_{j=1}^{t-1}M_i^j/HW$, where $M_i^j$ represents the actual number of measurements allocated to the $i^{\text{th}}$ block during the $j^{\text{th}}$ stage. Moreover, the expected 
cumulative sampling rate up to the $t^{\text{th}}$ sampling stage is set to $ts_\text{r}/N$. Thus, the expected sampling rate specifically for the $t^{\text{th}}$ stage $s_\text{r}^t=ts_\text{r}/N-\sum_i\sum_{j=1}^{t-1}M_i^j/HW$. Notably, by this stage, we already have the sampling results of the initial $t-1$ stages for each block. Therefore, we designed a measurement bounds prediction network that uses these sampling results to predict the measurement bounds of these blocks:
\begin{align}
g_{\boldsymbol{\theta}_m}\left(\left[{\textbf{\textit{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{t-1}}^\transpose, 0, \ldots, 0\right]^\transpose\right)=\hat{m}_i^t.
\end{align}
The measurement bounds prediction network $g_{\boldsymbol{\theta}_m}$ consists of several CNN layers and residual blocks \cite{He_2016_CVPR}, where $\boldsymbol{\theta}_m$ represents the network parameters.  $\textbf{\textit{y}}_i^1, \ldots, \textbf{\textit{y}}_i^{t-1}$ represent the sampling signals obtained from the first $t-1$ sampling stages for the $i^{\text{th}}$ block. Since the length of the concatenated sampling signal is likely to differ for each block, we pad zeros to the end of each concatenated sampling signal to ensure a consistent length of $B^2$. We compute the Kullback-Leibler (KL) Divergence-based loss to measure the discrepancy when the predicted measurement bounds $\hat{m}_i^t$ are employed to approximate the actual measurement bounds $m_i$, both in terms of distribution ratios, and use this KL divergence-based loss for network training:
\begin{align}
    \mathcal{L}_{\text{KL}}=\frac{1}{(N-1)\frac{HW}{B^2}}\sum_{t=2}^N\sum_i-\frac{m_i}{\sum_im_i}\log\frac{\hat{m}_i^t}{\sum_i\hat{m}_i^t}, 
    \label{eq:KL loss for measurement bounds prediction network training}
\end{align}
where the normalization factor of $\frac{1}{(N-1)\frac{HW}{B^2}}$ is chosen to average the loss over all sampling stages that have the step of predicting measurement bounds and over all blocks.

Once we obtain the predicted measurement bounds, we set the expected proportion of measurements allocated to the $i^{\text{th}}$ block after the $t^{\text{th}}$ stage as $p_i^t = \frac{\hat{m}_i^t}{\sum_i \hat{m}_i^t}$. However, the expected proportion is likely not achievable due to the fixed allocation ratios in the first $t-1$ stages. 

Once we have determined the allocation ratio $\{{q_i^t}^{\star}\}$, we can allocate the sampling rate and the number of measurements to the $i^\text{th}$ block based on this allocation ratio:
\begin{align}
    s_i^t & = \eta {q_i^t}^{\star}s_\text{r}^t\frac{HW}{B^2},\\
    M_i^t & = \round{s_i^tB^2}.
\end{align}
Here, $\eta$ plays a similar role as in \eqref{eq:distribute sampling rate}, its primary function being to align the actual sampling rate closely with the desired one. Next, we extract rows $\sum_{j=1}^{t-1}M_i^j+1$ through $\sum_{j=1}^{t}M_i^j$ from measurement matrix $\textit{\textbf{A}}$ to sample the $i^\text{th}$ block:
\begin{align}
    \textit{\textbf{y}}_i^t = \textit{\textbf{A}}_{\sum_{j=1}^{t-1}M_i^j+1:\sum_{j=1}^{t}M_i^j}\mathcal{V}(\textit{\textit{x}}_i).
\end{align}
After completing $N$ stages of sampling, we obtained the total number of measurements  as well as the final sampling result for the $i^{\text{th}}$ block:
\begin{align}
    M_i & = \sum_{j=1}^{N}M_i^j, \\
    \textit{\textbf{y}}_i & = \left[{\textit{\textbf{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{N}}^\transpose\right]^\transpose.
\end{align}

\subsubsection{Distribution Ratio Optimization}

Once we obtain the predicted measurement bounds, we set the expected proportion of measurements allocated to the $i^{\text{th}}$ block after the $t^{\text{th}}$ stage as $p_i^t = \frac{\hat{m}_i^t}{\sum_i \hat{m}_i^t}$. 
However, the expected proportion is likely not achievable due to the fixed allocation ratios in the first $t-1$ stages. Therefore, we can only adjust the allocation ratio for the current $t^{\text{th}}$ stage to make the actual cumulative allocation ratio over the first $t$ stages approximate the expected one.

To be specific, the proportion of measurements yet to be allocated in the current $t^{\text{th}}$ stage and the proportion of measurements allocated in the first $t-1$ stages, with respect to the total number of allocatable measurements in the first $t$ stages, are given by $\alpha^t = \frac{s_\text{r}^t}{ts_\text{r}/N}$ and $ \beta^t = 1 - \alpha^t = \frac{\sum_i\sum_{j=1}^{t-1}M_i^j/HW}{ts_\text{r}/N}$, respectively.
The fixed allocation ratio for the $i^{\text{th}}$ block is $r_i^t=\frac{\sum_{j=1}^{t-1}M_i^j}{\sum_i\sum_{j=1}^{t-1}M_i^j}$. Suppose the allocation ratio to be determined in the $t^{\text{th}}$ stage is $\{q_i^t\}$. Therefore, after the $t^{\text{th}}$ sampling stage, the actual allocation ratio is $\{\alpha^t q_i^t+\beta^t r_i^t\}$. We expect to adjust $\{q_i^t\}$ so that $\{\alpha^t q_i^t+\beta^t r_i^t\}$ is close to $\{p_i^t\}$ under the measurement of KL divergence-based object function. Additionally, $q_i^t$ is subject to upper and lower bounds. Clearly, the lower bound of $q_i^t$ is 0. Moreover, given that the number of measurements for the $i^{\text{th}}$ block must not exceed the length of its original signal, and considering that the count of measurements for the $i^{\text{th}}$ block at the $t^{\text{th}}$ sampling stage is approximately $q_i^ts_\text{r}^tHW$ (accounting for a rounding error), we can derive the following relationship:
\begin{align}
    q_i^ts_\text{r}^tHW + \sum_{j=1}^{t-1}M_i^j \leq B^2.
\end{align}
Therefore, we can obtain the upper bound of $q_i^t$, $a_i^t=\frac{B^2-\sum_{j=1}^{t-1}M_i^j}{s_\text{r}^tHW}$. Finally, we integrate the above considerations into a convex optimization problem:
\begin{equation}
\begin{aligned}
\argmin_{\{q_i^t\}} \quad  - & \sum_ip_i^t\log (\alpha^t q_i^t+\beta^t r_i^t) \\
\text{subject to} \quad & \sum_i q_i^t = 1, \\
                        & 0 \leq q_i^t \leq a_i^t \quad \text{for all} \quad i. 
\label{eq:allocation ratio optimization problem}                 
\end{aligned}
\end{equation}
We employ the Karush-Kuhn-Tucker (KKT) conditions to resolve this issue, with the solution procedure detailed in Appendix~\ref{appendix:solution}.

\paragraph{Solving the Lagrange Multipliers}

Building on our earlier discussion, we have derived the closed-form solution of the convex optimization problem as: ${q_i^t}^{\star} = \min\left(\max\left(\frac{p_i^t}{\nu^{\star}} - \frac{\beta^t r_i^t}{\alpha^t}, 0\right), a_i^t\right)$. The next step is to identify the value of the Lagrange multiplier $\nu^{\star}$ in order to determine the solution for ${q_i^t}^{\star}$. To simplify our notation, we substitute $\nu^\star$ with $\frac{1}{\mu^\star}$ (based on the conclusion in Appendix~\ref{appendix:solution} that $\nu^\star > 0$, we only consider cases where $\mu^\star > 0$). This leads us to rewrite the closed-form solution of the convex optimization problem as:
\begin{align}
{q_i^t}^{\star} = \min\left(\max\left(\mu^{\star}p_i^t - \frac{\beta^t r_i^t}{\alpha^t}, 0\right), a_i^t\right).
\label{eq:distribution ratio optimization}
\end{align}
Define $Q_i^t(\mu) = \min\left(\max\left(\mu p_i^t- \frac{\beta^t r_i^t}{\alpha^t}, 0\right), a_i^t\right)$, and let $Q^t(\mu) = \sum_i Q_i^t(\mu)$. Based on the constraint condition in \eqref{eq:allocation ratio optimization problem} that the sum of the allocation ratios should be equal to 1, our problem is transformed into finding $\mu$ that satisfies $Q^t(\mu) = 1$.

Before examining the function $Q^t(\mu)$, let us first define some notation: $N_\text{l}^t(\mu)=\{i|Q_i^t(\mu)=0\}$, $N_\text{c}^t(\mu)=\{i|0<Q_i^t(\mu)<a_i^t\}$ and $N_\text{u}^t(\mu)=\{i|Q_i^t(\mu)=a_i^t\}$. With the help of this notation, we obtain another representation of $Q^t(\mu)$:
\begin{align}
    Q^t(\mu) = \sum_i Q_i^t(\mu) &= \sum_{i\in N_\text{c}^t(\mu)}(\mu p_i^t - \frac{\beta^t r_i^t}{\alpha^t}) + \sum_{i\in N_\text{u}^t(\mu)}a_i^t.
\end{align}
The derivative of $Q^t(\mu)$ with respect to $\mu$ can be formulated as:
\begin{align}
    {Q^t}'(\mu) &= \sum_{i\in N_\text{c}^t(\mu)}p_i^t.
\end{align}
The function $Q^t(\mu)$ should be a piecewise linear monotonically increasing function with its domain being $(0, +\infty)$ and its range being $[0, \sum_{i=1}^n a_i^t]$. The boundary points of each linear segment correspond to those points $\mu$ that cause changes in $\{N_\text{J}(\mu) | \text{J} = \text{l}, \text{c}, \text{u}\}$. Fig.~\ref{fig:the approximate shape of Q(mu)} shows the approximate shape of the $Q^t(\mu)$ function.
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{Figures/Qmu.png}
    \caption{The approximate graphical representation of the function $Q^t(\mu)$.}
    \label{fig:the approximate shape of Q(mu)}
\end{figure}

Next, our goal is to locate the root of $Q^t(\mu)=1$ utilizing Newton's method. The principle behind Newton's method is that at each iteration, the algorithm finds an updated approximation of the root under the assumption that the function behaves as locally linear around the current approximation. Specifically, in the $\tau^{\text{th}}$ iteration, we have:
\begin{align}
    1&=(\mu^{(\tau+1)}-\mu^{(\tau)}){Q^t}'(\mu^{(\tau)})+Q^t(\mu^{(\tau)}),
\end{align}
where $\mu^{(\tau)}$ is the result of the $\tau^{\text{th}}$ iteration of Newton's method. By relocating $\mu^{(\tau+1)}$ to the left side of the equation and shifting the other terms to the right side, we obtain:
\begin{align}
    & \mu^{(\tau+1)} = \frac{1-Q^t(\mu^{(\tau)})}{{Q^t}'(\mu^{(\tau)})}+\mu^{(\tau)} \nonumber \\
    & =\frac{1-\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}(\mu^{(\tau)}p_i^t-\frac{\beta^t r_i^t}{\alpha^t})-\sum_{i\in N_\text{u}^t(\mu^{(\tau)})}a_i^t}{\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}p_i^t}+\mu^{(\tau)} \nonumber \\
    & =\frac{1+\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}\frac{\beta^t r_i^t}{\alpha^t}-\sum_{i\in N_\text{u}^t(\mu^{(\tau)})}a_i^t}{\sum_{i\in N_\text{c}^t(\mu^{(\tau)})}p_i^t}. \label{eq:newton_iter}
\end{align}
In general, both the numerator and the denominator in the last expression of \eqref{eq:newton_iter} are greater than zero, unless the initial value for Newton's method is set too small or too large. Empirically, setting $\mu^{(0)} = \frac{\beta^t}{\alpha^t}$ ensures both are positive. We set the termination condition as $\{N_\text{J}^t(\mu^{(\tau)}) | \text{J} = \text{l}, \text{c}, \text{u}\}$ being entirely equal to $\{N_\text{J}^t(\mu^{(\tau+1)}) | \text{J} = \text{l}, \text{c}, \text{u}\}$, that is, $\mu^{(\tau)}$ and $\mu^{(\tau+1)}$ are in the same linear function segment. In this case, we can deduce that $\mu^{(\tau+1)}$ is the root of $Q^t(\mu) = 1$:
\begin{equation}
\begin{aligned}
    Q^t(\mu^{(\tau+1)}) & = \sum_{i\in N_\text{c}^t(\mu^{(\tau+1)})}(\mu^{(\tau+1)}p_i^t - \frac{\beta^t r_i^t}{\alpha^t}) + \sum_{i\in N_\text{u}^t(\mu^{(\tau+1)})}a_i^t \\
    & = \sum_{i\in N_\text{c}^t(\mu^{(\tau)})}(\mu^{(\tau+1)}p_i^t - \frac{\beta^t r_i^t}{\alpha^t}) + \sum_{i\in N_\text{u}^t(\mu^{(\tau)})}a_i^t \\
    & \stackrel{\text{According to \eqref{eq:newton_iter}}}{=}1. \nonumber
\end{aligned}
\end{equation}

Subsequently, we wish to consider the convergence issue of Newton's method under discussion. The difficulty in directly referencing previous methods of proving the convergence of Newton's method is that the general Newton's method deals with smooth functions, and considers the convergence speed of the error upper bound as $\tau$ increases. However, in this specific scenario, during the Newton's iteration process, $\mu^{(\tau)}$ will fall into different linear segments, until $\mu^{(\tau)}$ falls into the linear segment identical to the root (as stated above, once we find the linear segment where the root is located, we can obtain the root through one iteration of Newton's method). From this perspective, this problem is concerned with finding the root's linear segment from all possible linear segments, rather than focusing on the convergence speed of the error in the solution. Consequently, we are currently seeking to propose a fallback plan for when Newton's method fails to converge, ensuring that we eventually identify the linear segment hosting the root.

To manage scenarios where Newton's method fails to converge, we first present Lemma \ref{lemma:inequality relationship} in Appendix~\ref{appendix:lemma}. This lemma allows us to understand the interval in which $\mu^\star$ is located and assists us further narrow down this interval. Specifically, we can determine the upper and lower bounds of $\mu^\star$ by comparing the relationship between $\mu^{(\tau)}$ and $\mu^{(\tau+1)}$. For example, if $\mu^{(\tau)} < \mu^{(\tau+1)}$, based on Lemma \ref{lemma:inequality relationship}, we can deduce that $\mu^{(\tau)} < \mu^{\star}$. Then, compare $\mu^{(\tau)}$ with the existing lower bound; if $\mu^{(\tau)}$ is greater than the current lower bound, update the lower bound to $\mu^{(\tau)}$.

\input{Section/proposed_method_subsection/newton_and_bisection_algorithm}

Next, we can assess the convergence at each iteration of Newton's method by using the upper and lower bounds obtained from Lemma \ref{lemma:inequality relationship}. 
If the result of a particular iteration surpasses the upper or lower bound, we consider that this iteration has not converged. Therefore, we utilize the bisection method to replace the result of this iteration by the average of the lower and upper bounds. Even if all iterations in Newton's method fail to converge, we can still use Lemma \ref{lemma:inequality relationship} to ascertain whether the root is smaller or larger than our current result. This helps define the bisection method's search interval, guiding the overall process to locate the linear segment where the root lies via bisection method instead of Newton's method. We have developed Algorithm \ref{alg:find root with newton's method and bisection method} based on this methodology. For the sake of convenient notation, we have removed the superscript $t$ that indicates the stage number. Additionally, the function $\chi_\textbf{\textit{b}}(\bm{\omega}):\mathbf{R}^{\frac{HW}{B^2}} \rightarrow \mathbf{R}^{\frac{HW}{B^2}}$($\textbf{\textit{b}}\in \mathbf{R}^{\frac{HW}{B^2}}$) is specified as:
\begin{align}
\chi_\textbf{\textit{b}}(\bm{\omega})_i= \begin{cases} 1 & \text{if } \omega_i=b_i \\ 0  & \text{if } \omega_i\neq b_i
\end{cases}
\end{align}

\paragraph{Distribution of Measurements}

Once we have determined the allocation ratio $\{{q_i^t}^{\star}\}$, we can allocate the sampling rate and the number of measurements to the $i^\text{th}$ block based on this allocation ratio:
\begin{align}
    s_i^t & = \eta {q_i^t}^{\star}s_\text{r}^t\frac{HW}{B^2},\\
    M_i^t & = \round{s_i^tB^2}.
\end{align}
Here, $\eta$ plays a similar role as in \eqref{eq:distribute sampling rate}, its primary function being to align the actual sampling rate closely with the desired one. Next, we extract rows $\sum_{j=1}^{t-1}M_i^j+1$ through $\sum_{j=1}^{t}M_i^j$ from measurement matrix $\textit{\textbf{A}}$ to sample the $i^\text{th}$ block:
\begin{align}
    \textit{\textbf{y}}_i^t = \textit{\textbf{A}}_{\sum_{j=1}^{t-1}M_i^j+1:\sum_{j=1}^{t}M_i^j}\mathcal{V}(\textit{\textit{x}}_i).
\end{align}
After completing $N$ stages of sampling, we obtained the total number of measurements  as well as the final sampling result for the $i^{\text{th}}$ block:
\begin{align}
    M_i & = \sum_{j=1}^{N}M_i^j, \\
    \textit{\textbf{y}}_i & = \left[{\textit{\textbf{y}}_i^1}^\transpose, \ldots, {\textbf{\textit{y}}_i^{N}}^\transpose\right]^\transpose.
\end{align}


==> Section/related_work_old.tex <==
\section{Related Works}\label{sec:related_work}
To our knowledge, current CS methods can be divided into optimization-based methods and data-driven methods. In this section, we will introduce these two types of methods respectively, and provide a detailed discussion on the works related to our method.

\subsection{Optimization-based Methods}
Traditional CS, which follows a optimization-based method, usually defines the problem of reconstructing the original signal $\textbf{\textit{x}}$ from the known sampled signal $\textbf{\textit{y}}$ as an optimization problem (often a convex optimization problem):
\begin{align}
    \hat{\textbf{\textit{x}}} = \argmin_{\textbf{\textit{x}}} \|\boldsymbol{\Phi} \textbf{\textit{x}}-\textbf{\textit{y}}\|_2^2 + \lambda \mathcal{R}(\textbf{\textit{x}}),
\end{align}

where $\mathcal{R}$ denotes a particular prior regularization or a set of them, while $\lambda$ represents the weight of this regularization.

The common methods to solve this optimization problem include: convex optimization methods \cite{doi:10.1137/S003614450037906X}, greedy algorithms \cite{258082}, and gradient descent methods\cite{f957882f5b1e4f3ba0450468093903f1}. 

For the problem of image CS, some studies have proposed incorporating image priors into the regularization term of the optimization problem. \cite{li2013efficient} introduces total variation to represent local smoothness priors, replacing sparsity priors. \cite{5414429} advocates for sparsity and smoothness in the domain of directional transforms for images. \cite{6341094} presents a collaborative sparsity method, which simultaneously imposes local 2-D and nonlocal 3-D sparsity in an adaptable hybrid domain. \cite{6814320} suggests a group-based sparse representation model, considering inter-patch relationships and adaptively inducing sparsity in natural images within group domains. Additionally, there are some articles that consider improving CS from other perspectives. \cite{4288604} proposes a block CS framework for natural images to capture complicated geometric structures. \cite{6190204} proposes to utilize multihypothesis predictions to generate a residual in the domain of CS random projections.

\subsection{Data-driven Methods}
In recent years, many studies have focused on integrating data-driven methods with CS, achieving commendable reconstruction quality and speed. \cite{Kulkarni_2016_CVPR} proposed the use of CNN to learn the reconstruction from sampled signals to original signals. \cite{8765626} suggested an end-to-end sampling-reconstruction structure, employing CNN to eliminate block effects caused by block sampling. \cite{Zhang_2018_CVPR} replaced the sparsity constraint in the linear transform domain in the traditional optimization-based unfolding algorithm, Iterative Shrinkage-Thresholding Algorithm (ISTA) \cite{doi:10.1137/080716542}, with the sparsity constraint in the network-based nonlinear transform domain. Combining data-driven ideas with traditional unfolding methods has further enhanced model performance. \cite{9019857} continued this approach and explored inter-block relationships. \cite{9298950} extended another unfolding algorithm, AMP, into a network structure. \cite{9934025} proposed introducing Transformers into the reconstruction network to enhance its capacity to model long-distance relationships.
     
Some studies consider the design of deep CS models from other perspectives: the scalability of the model (including the scalability for sampling ratios and measurement matrices) and the adaptive allocation of sampling ratios. \cite{Shi_2019_CVPR} aims to design a model that adapts to different sampling ratios with a single model. It achieves scalability from coarse-grain to fine-grain sampling ratios by employing a hierarchical network structure and a greedy algorithm for selecting measurement bases. \cite{9467810} introduced a controllable arbitrary-sampling network method named COAST, which solves the CS problem of any sampling matrix with a single model through a random projection augmentation strategy. \cite{5585813} proposed using the Pulsed Cosine Transform (PCT) to mimic neuronal pulses in the human brain to generate saliency maps to guide the adaptive allocation of sampling ratios. Although this method can distinguish which areas are more important to human perception, it cannot rigorously specify and prove what kind of mapping relationship should exist between the importance of an area and the proportion of sampling ratio. \cite{9854112} proposed a more efficient network-based saliency map generator for learning adaptive sampling ratio allocation strategy. However, the task of allocating measurements to each block is a high-dimensional discrete optimization problem. This network-based method expands this problem into a continuous optimization problem, making the problem derivable for backpropagation. Yet, the network-based approach, which usually seeks the local optimal solution of the continuous problem through gradient updates, may not necessarily converge to the global optimum of the original high-dimensional discrete problem.
   

==> Section/related_work_old2.tex <==
\section{Related Works}\label{sec:related_work}
CS belongs to a category of inverse problems. Broadly speaking, inverse problems in images encompass a variety of challenges, including but not limited to super-resolution \cite{9426447, zhou2023memory, 10314443}, denoising \cite{8852852, 7577781, 6307863}, deblurring \cite{10274681, cui2023dual, zhang2022deep},  deraining \cite{li2021comprehensive, 10122854, 10120722}, low-light enhancement \cite{8692732, 9741357, 10102793}, and CS. constructSpecifically, current CS methods can be divided into optimization-based methods and data-driven methods. In this section, we will introduce them respectively, and provide a detailed discussion on the works related to our method.

\subsection{Optimization-based Methods}
Traditional CS, which follows an optimization-based method, usually defines the problem of reconstructing the original signal $\textbf{\textit{x}}$ from the known sampled signal $\textbf{\textit{y}}$ as an optimization problem:
\begin{align}
    \hat{\textbf{\textit{x}}} = \argmin_{\textbf{\textit{x}}} \|\boldsymbol{\Phi} \textbf{\textit{x}}-\textbf{\textit{y}}\|_2^2 + \lambda \mathcal{R}(\textbf{\textit{x}}),
\end{align}
where $\mathcal{R}$ denotes a regularization term that capture task-dependent prior knowledge, while $\lambda$ represents the weight of this regularization.

The common methods to solve this optimization problem include: convex optimization methods \cite{doi:10.1137/S003614450037906X}, greedy algorithms \cite{258082}, and gradient descent methods \cite{f957882f5b1e4f3ba0450468093903f1}. 

For image CS, some studies have proposed incorporating image priors into the regularization term. \cite{li2013efficient} introduces total variation to represent local smoothness priors, replacing sparsity priors. \cite{5414429} advocates for sparsity and smoothness in the domain of directional transforms for images. \cite{6341094} presents a collaborative sparsity method, which simultaneously imposes local 2-D and nonlocal 3-D sparsity in an adaptable hybrid domain. \cite{6814320} suggests a group-based sparse representation model, considering inter-patch relationships and adaptively inducing sparsity in natural images within group domains. \cite{7923735} proposes an adaptive bandwise sparsity regularization with patch-specific adaptive PCA for quantized CS.

\subsection{Data-driven Methods}
In recent years, many studies have focused on integrating data-driven methods with CS, achieving commendable reconstruction quality and speed. \cite{Kulkarni_2016_CVPR} proposed the use of CNN to learn the reconstruction from sampled signals to original signals. \cite{8765626} suggested an end-to-end sampling-reconstruction structure, employing CNN to eliminate block effects caused by block sampling. \cite{Zhang_2018_CVPR} replaced the sparsity constraint in the linear transform domain in the traditional optimization-based unfolding algorithm, Iterative Shrinkage-Thresholding Algorithm (ISTA) \cite{doi:10.1137/080716542}, with the sparsity constraint in the network-based nonlinear transform domain. Combining data-driven ideas with traditional unfolding methods has further enhanced model performance. \cite{9019857} continued this approach and explored inter-block relationships. \cite{9298950} extended another unfolding algorithm, AMP, into a network structure. \cite{9934025} proposed introducing Transformers \cite{NIPS2017_3f5ee243} into the reconstruction network to enhance its capacity to model long-distance relationships.
     
Some studies consider the design of deep CS models from other perspectives: the scalability of the model (including the scalability for sampling rates and measurement matrices) and the adaptive allocation of sampling rates across different image blocks. \cite{Shi_2019_CVPR} aims to design a model that adapts to different sampling rates with a single model. It achieves scalability from coarse to fine-grained sampling rates by employing a hierarchical network structure and a greedy algorithm for selecting measurement bases. \cite{9467810} introduced a controllable arbitrary-sampling network method named COAST, which solves the CS problem of any sampling matrix with a single model through a random projection augmentation strategy. \cite{5585813} proposed using the Pulsed Cosine Transform (PCT) to mimic neuronal pulses in the human brain to generate saliency maps to guide the adaptive allocation of sampling rates. Although this method can distinguish which areas are more important to human perception, it cannot rigorously specify and prove what kind of mapping relationship should exist between the importance of an area and the proportion of sampling rate. \cite{9854112} proposed a more efficient network-based saliency map generator for learning adaptive sampling rate allocation strategy. The task of allocating measurements, which is originally a high-dimensional discrete optimization problem, is transformed into a continuous problem and the parameters of the network used for allocating measurements are updated via backpropagation. However, this approach may only find a local optimum rather than the global optimum of the original high-dimensional discrete problem, and have limitations in robustness and generalizability.
   
